Synthetic Interventions

The synthetic controls (SC) methodology is a prominent tool for policy evaluation in panel data applications. Researchers commonly justify the SC framework with a low-rank matrix factor model that assumes the potential outcomes are described by low-dimensional unit and time specific latent factors. In the recent work of [Abadie '20], one of the pioneering authors of the SC method posed the question of how the SC framework can be extended to multiple treatments. This article offers one resolution to this open question that we call synthetic interventions (SI). Fundamental to the SI framework is a low-rank tensor factor model, which extends the matrix factor model by including a latent factorization over treatments. Under this model, we propose a generalization of the standard SC-based estimators. We prove the consistency for one instantiation of our approach and provide conditions under which it is asymptotically normal. Moreover, we conduct a representative simulation to study its prediction performance and revisit the canonical SC case study of [Abadie-Diamond-Hainmueller '10] on the impact of anti-tobacco legislations by exploring related questions not previously investigated.

==> content/SC_case_studies.tex <==

\subsection{Subspace Inclusion Test Applied to Synthetic Controls}\label{ssec:case-studies}
%
We revisit two seminal case studies within the SC literature: 
%
(i) an evaluation on the impact of terrorism in Basque Country \cite{abadie1}; 
%
(ii) an evaluation on the impact of California's Proposition 99 on tobacco consumption \cite{abadie2}. 
%
In particular, we apply our subspace inclusion hypothesis test to study the potential feasibility of counterfactual inference in both studies.
%
Indeed, these studies have been used extensively to explain the utility of the SC method and have subsequently served as benchmarks in following works, cf. \cite{rsc, athey1, ark, agarwal2020robustness}, and more broadly as well.
%
As such, we hope our findings not only motivate the usage of this test, but also spark the development of additional robustness tests to stress test the causal conclusions drawn from these studies and beyond. 


\subsubsection{Terrorism in Basque Country} 
%
\noindent {\em Background \& setup.} 
%
In 1968, the first Basque Country victim of terrorism was claimed; however, it was not until the mid-1970s 
did the terrorist activity become more rampant \cite{abadie1}. 
%
To study the economic ramifications of 
terrorism on Basque Country, we use the per-capita GDP of $N=18$ Spanish regions from 1955-1997, i.e., $T=43$. 
%
Among these regions, there is one treated region, Basque Country, which experienced terrorism; the other 17 regions are considered control regions as they were relatively unaffected by terrorism. 
%
Translating to our notation, we have $D=2$ with $d=0$ representing control and $d=1$ representing treatment (i.e., terrorism); 
%
in turn, we have $T_0 = 14$ and $T_1 = 29$. 
%
Without loss of generality, we index Basque Country as unit $n=1$. 
%
Our interest is to estimate $\theta^{(0)}_1$. 

We note that the original work of \cite{abadie1} uses 13 additional predictor variables for each region, including demographic information pertaining to one's educational status, and average shares for six industrial sectors.
%
We do not utilize this additional information here, i.e., we only use information related the outcome of interest, i.e., per-capita GDP.


\vspace{10pt} \noindent 
{\em Hypothesis test results.} 
%
We apply our heuristic variant of the hypothesis test, introduced in Section~\ref{sec:practical_heuristic}, with $\alpha = 0.05$. 
%
We find that our test statistic  
$\htau = 0.01$ and $\tau(\alpha) = 0.05$. 
%
Since $\htau < \tau(\alpha)$, our tests suggest that the SI method is suitable for this study, and also supports the suitability of and conclusions drawn from previous works utilizing SC-like methods for this case study.

\subsubsection{California Proposition 99} 
%
\noindent {\em Background \& setup.} 
%
In 1988, California introduced the 
first modern large-scale anti-tobacco legislation in the United States \cite{abadie2}. 
%
To analyze the effect of California's anti-tobacco legislation, we use the annual per-capita cigarette consumption at the state level for $N=39$ states from 1970-2000, i.e., $T=31$. 
%
With the exception of California, the other 38 states included in this study neither adopted an anti-tobacco program or raised cigarette sales taxes by 50 cents or more.
%
As such, these states are considered the control states and California is considered the treated state. 
%
Translating to our notations, we have $D=2$ with $d=0$ representing control and $d=1$ representing treatment (i.e., Proposition 99); 
in turn, we have $T_0 = 29$ and $T_1 = 12$. 
%
Without loss of generality, we index California as unit $n=1$. 
%
Our interest is to estimate $\theta^{(0)}_1$.  
 
It is worth noting that the original work in \cite{abadie2} uses six additional covariates per state, e.g., retail price, 
beer consumption per capita, and percentage of individuals between ages of 15-24. 
% 
We do not include these variables in our study. 

\vspace{10pt} \noindent {\em Hypothesis test results.} 
%
We apply our heuristic variant of the hypothesis test with $\alpha = 0.05$. %
We find that our test statistic  
$\htau = 1.64$ and $\tau(\alpha) = 0.15$. 
%
Since $\htau > \tau(\alpha)$, our test suggests that the SI estimator is likely ill-suited to produce a reliable estimate of $\theta^{(0)}_1$; 
in fact, our test only passes for $\alpha \ge 0.48$. 
%
Since the robust synthetic controls estimator of \cite{rsc, agarwal2020robustness} is a special case of the SI estimator, this puts into question the conclusions drawn in \cite{rsc, agarwal2020robustness}. 
%
More generally, this may shed some doubt on the suitability of any linear predictor, including the original SC estimator and many of its variants (e.g. \cite{athey1, ark}), used to investigate the impact of Proposition 99.
%
Thus, we believe this result may be of independent interest to the SC literature to revisit the conclusions drawn from these prior works and to further extend the toolkit of robustness/sensitivity analysis tests of when one can transfer a model across time periods (and interventional regimes).


% In turn, this puts into question the suitability of any linear predictor, including the original synthetic controls estimator and many of its variants, and thus the conclusions drawn in associated prior works, \cite{abadie2, amjad, ark} to name a few. 

% \begin{figure}
% 	\centering
% 	\begin{subfigure}[b]{0.45\textwidth}
% 		\centering
% 		\includegraphics[width=\textwidth]{prop99_spectra.png}
% 		\caption{Spectra of California smoking control data.}
% 		\label{fig:cali_eig}
% 	\end{subfigure}
% 	\hfill 
% 	\begin{subfigure}[b]{0.45\textwidth}
% 		\centering
% 		\includegraphics[width=\textwidth]{basque_spectrum.png}
% 		\caption{Spectra of Basque Country control data.}
% 		\label{fig:basque_eig}
% 	\end{subfigure}
% 	\caption{}
% 	\label{fig:sc_spectra}
% \end{figure}

==> content/helper_lemmas.tex <==
\subsection{Helper Lemmas}

% helper lemma
\begin{lemma} \label{lemma:trace.1} 
Let $\bA, \bB \in \Rb^{n \times n} $ be symmetric PSD matrices. Then, $\tr(\bA \bB) \ge 0$. 
\end{lemma} 

\begin{proof}
Let $\bB^{1/2}$ denote the square root of $\bB$. Since $\bA \succeq 0$, we have
$
	\tr(\bA \bB) = \tr(\bA \bB^{1/2} \bB^{1/2})
	= \tr(\bB^{1/2} \bA \bB^{1/2}) %
	= \sum_{i=1}^n (\bB^{1/2} e_i)^\prime \bA  (\bB^{1/2} e_i) \ge 0,
$ 
\end{proof} 

 \begin{lemma} \label{lemma:trace.2} 
If $\bA \in \Rb^{n \times n}$ is a symmetric matrix and $\bB \in \Rb^{n \times n}$ is a symmetric PSD matrix, then
$
	\tr(\bA \bB) \le \lambda_{\max}(\bA) \cdot \tr(\bB),
$
where $\lambda_{\max}(\bA)$ is the top eigenvalue of $\bA$. 
\end{lemma} 

\begin{proof}
Since $\bA$ is symmetric, it follows that  
$\lambda_{\max}(\bA) \bI - \bA \succeq 0$. 
As a result, applying Lemma \ref{lemma:trace.1} yields
$
	\tr((\lambda_{\max}(\bA) \bI - \bA) \bB) = \lambda_{\max}(\bA) \cdot \tr(\bB) - \tr(\bA \bB) \ge 0. 
$
%This completes the proof. 
\end{proof}

==> content/hypothesis_test.tex <==
\section{A Hypothesis Test for Subspace Inclusion} \label{sec:hypo} 
%
In Section \ref{sec:hypothesis.test}, we formally define the subspace inclusion hypothesis test; this serves as a robustness check of Assumption \ref{assumption:subspace}, which enables our learned model to be transferred across interventions and measurements.
%
In Section \ref{ssec:case-studies}, we apply this test to two seminal case studies from the SC literature and discuss our findings.


\subsection{Hypothesis Test \& Formal Results}\label{sec:hypothesis.test}
%
\noindent
%
{\em Notation.}
%
Recall $r_\pre = \rank(\Ex[\bY_{\pre, \Ic^{(d)}}])$ and $r_\post = \rank(\Ex[\bY_{\post, \Ic^{(d)}}])$. 
%
Further, recall $\bV_\pre \in \Rb^{N_d \times r_\pre}$ denotes the right singular vectors of $\Ex[\bY_{\pre, \Ic^{(d)}}]$. 
%
Define $\bV_\post \in \Rb^{N_d \times r_\post}$ with respect to $\Ex[\bY_{\post, \Ic^{(d)}}]$ analogously. 
%
Finally, let $\bhV_\pre \in \Rb^{N_d \times r_\pre}$ and $\bhV_\post \in \Rb^{N_d \times r_\post}$ denote their respective estimates, which are constructed from the top $r_\pre$ and $r_\post$ right singular vectors of $\bY_{\pre, \Ic^{(d)}}$ and $\bY_{\post, \Ic^{(d)}}$, respectively. 

\subsubsection{Hypothesis Test}\label{ssec:hypo_}
%
Consider hypotheses
\begin{align}
	H_0: ~ \tspan(\bV_\post) \subseteq \tspan(\bV_\pre)
	\quad \text{and} \quad 
	H_1: ~ \tspan(\bV_\post) \nsubseteq \tspan(\bV_\pre).
\end{align}
Recall the test statistic $\htau$ as defined in \eqref{eq:test_stat} in Section \ref{sec:si_algo_hypo_test}. 
% %
% Consider the noiseless case (i.e., $\varepsilon^{(d)}_{tn} = 0$), where $\bV_\pre$ and $\bV_\post$ are perfectly observed.
% %
% Conditioned on $H_0$, note that $\|(\bI - \bV_\pre \bV_\pre^\prime)\bV_\post\|_F = 0$, while conditioned on $H_1$, $\|(\bI - \bV_\pre \bV_\pre^\prime)\bV_\post\|_F > 0$.
% %
% Hence, $\|(\bI - \bV_\pre \bV_\pre^\prime)\bV_\post\|_F$ serves as a natural test statistic. 
% %
% Since we do not observe these quantities, we use $\bhV_\pre$ and $\bhV_\post$ as proxies.
% %
More formally, we define the test as follows: for any significance level $\alpha \in (0,1)$,
%
\begin{align}
	\text{Retain } H_0 \text{ if } ~\htau \le \tau(\alpha)
	\quad \text{and} \quad  \text{Reject } H_0 \text{ if } ~\htau > \tau(\alpha).
\end{align}
%
Here, $\tau(\alpha)$ is the critical value, which we define for some absolute constant $C \ge 0$: 
%
\begin{align}\label{eq:crit_value}
%
\tau(\alpha) &= 
%
\frac{C\sigma^2 r_\post \phi^2_\pre(\alpha/2)}{s^2_{r_\pre}}
%
+ \frac{C\sigma^2 r_\post \phi^2_\post(\alpha/2)}{\varsigma^2_{r_\post}}
%
+ \frac{C\sigma r_\post \phi_\pre(\alpha/2)}{s_{r_\pre}}, 
%
\end{align}
%
where $\phi_\pre(a) = \sqrt{T_0} + \sqrt{\numdonors} + \sqrt{\log(1/a)}$;
%
$\phi_\post(a) = \sqrt{T_1} + \sqrt{\numdonors} + \sqrt{\log(1/a)}$;  and 
$s_\ell, \varsigma_\ell$ are the $\ell$-th singular values of 
$\Ex[ \bYpred | \cE]$ and $\Ex[ \bYpostd | \cE]$, respectively. 
%

\subsubsection{Type I and Type II Error Guarantees} 
%
Given our choice of $\htau$ and $\tau(\alpha)$, we control both Type I and Type II 
errors of our test. 
%
\begin{thm} \label{thm:hypo}
%
Let Assumptions \ref{assumption:sutva},  \ref{assumption:form}, \ref{assumption:conditional_mean_zero},  \ref{assumption:noise} hold. 
%
Fix any $\alpha \in (0,1)$. 
%
Then conditioned on $\Ec$, there exists an absolute constant $C \ge 0$, defined in \eqref{eq:crit_value}, such that 
% 
the Type I error is bounded as 
%
$
\Pb(\htau > \tau(\alpha) | H_0) \le \alpha. 
$
%
To bound the Type II error, suppose the following additional condition holds:
\begin{align} \label{eq:type2_cond} 
    r_\epost > \| \bV_\epre \bV_\epre^\prime \bV_\epost \|_F^2 
    + 2 \tau(\alpha) + 
    \frac{C\sigma r_\epost \phi_\epost(\alpha/2)}{\varsigma_{r_\epost}}.
\end{align}
% which implies $H_1$ must hold. 
%
Then, the Type II error is bounded as 
$
\Pb(\htau \le \tau(\alpha) | H_1) \le \alpha.
$
\end{thm}
%
The particular $C$ for which Theorem \ref{thm:hypo} holds depends on the underlying distribution of $\varepsilon^{(d)}_{tn}$, which determines the distribution of the potential outcomes $Y^{(d)}_{tn}$. 
%
$C$ can be made explicit for certain classes of distributions; as an example, Corollary \ref{cor:hypo} specializes Theorem \ref{thm:hypo} to when $\varepsilon^{(d)}_{tn}$ are normally distributed. 
%
\begin{cor}\label{cor:hypo}
%
Consider the setup of Theorem \ref{thm:hypo} with $C=4$.  
%
Let $\varepsilon^{(d)}_{tn}$ be normally distributed for all $(t,n,d)$. 
%
Then, $\Pb(\htau > \tau(\alpha) | H_0) \le \alpha$ and  $\Pb(\htau \leq \tau(\alpha) | H_1) \le \alpha.$
\end{cor}
%
We now argue \eqref{eq:type2_cond} is not a restrictive condition.
%
Conditioned on $H_1$, observe that $ r_\post > \|\bV_\pre \bV_\pre^\prime \bV_\post \|_F^2$ always holds. 
%
If Assumption \ref{assumption:spectra} holds and the nonzero singular values of $\Ex[\bY_{\post, \Ic^{(d)}}]$ are well-balanced, then one can easily verify that the latter two terms on the right-hand side of \eqref{eq:type2_cond} decay to zero as $T_0, T_1, N_d$ grow.


\subsubsection{Computing $\tau(\alpha)$} \label{sec:computing_tau} 
%
Computing $\tau(\alpha)$ requires estimating (i) $\sigma^2$;  (ii) $r_\pre, r_\post$; (iii) $s_{r_\pre}, \varsigma_{r_\post}$. 
%
We provide an estimator for $\sigma$ in \eqref{eq:hat_sigma} and establish its consistency in Theorem~\ref{thm:normality}. 
%
Further, recall that Lemma \ref{lemma:singular_values} establishes that the singular values of $\bY_{\pre, \Ic^{(d)}}$ and $\Ex[\bY_{\pre, \Ic^{(d)}}]$ must be close.
%
Thus, we can use the spectra of $\bY_{\pre, \Ic^{(d)}}$ as a good proxy to estimate $r_\pre$ and $s_{r_\pre}$.
%
Analogous arguments hold for $\bY_{\post, \Ic^{(d)}}$ with respect to $\Ex[\bY_{\post, \Ic^{(d)}}]$.
%
Further, note that Corollary \ref{cor:critical_value} specializes $\tau(\alpha)$ under Assumption \ref{assumption:spectra}. 
%
\begin{cor}\label{cor:critical_value}
%
Let the setup of Theorem \ref{thm:hypo} hold.
%
Suppose Assumption \ref{assumption:spectra} holds.
%
Further, suppose that conditioned on $\cE$, the $r_{\epost}$ nonzero singular values $\varsigma_i$ of $\Ex[\bY_{\epost, \Ic^{(d)}}]$ are well-balanced, i.e., $\varsigma_i^2 = \Theta(T_1 \numdonors / r_{\epost})$. 
%
Then, $\tau(\alpha) = O\Big( \frac{\sqrt{\log(1 / \alpha)}}{\min\{\sqrt{T_0}, \sqrt{T_1}, \sqrt{\numdonors} \}} \Big).$
%
\end{cor} 
%
If we consider the noiseless case, $\varepsilon^{(d)}_{tn} = 0$, we note that $\tau(\alpha) = 0$.
%
More generally, if the spectra of $\Ex[\bY_{\pre, \Ic^{(d)}}]$ and $\Ex[\bY_{\post, \Ic^{(d)}}]$ are well-balanced, then Corollary \ref{cor:critical_value} establishes that $\tau(\alpha) = o(1)$, even in the presence of noise. 
%
We remark that Corollary \ref{cor:hypo} allows for exact constants in the definition of $\tau(\alpha)$ under the Gaussian noise model.  

\subsubsection{A Practical Heuristic} \label{sec:practical_heuristic} 
%
Here, we provide a complementary approach to computing $\tau(\alpha)$, 
used in \cite{squires2021causal}.
%
To build intuition, observe that $\htau$ represents the remaining spectral energy of $\bhV_\post$ not contained within $\text{span}(\bhV_\pre)$. 
%
Further, we note $\htau$ is trivially bounded by $r_\post$ since the columns of $\bhV_\post$ are orthonormal. 
%
Thus, one can fix some fraction $\alpha \in (0,1)$ and reject $H_0$ if $\htau > \tau(\alpha)$, where $\tau(\alpha) = \alpha \cdot r_\post$. 
%
In words, if more than $\alpha$ fraction of the spectral energy of $\bhV_\post$ lies outside the span of $\bhV_\pre$, then the alternative test rejects $H_0$. 
%
We remark that this variant is likely more robust compared to its exact computation counterpart, which requires estimating several ``nuisance'' quantities described above in order to estimate \eqref{eq:crit_value} and varies with the underlying modeling assumptions we make about $\varepsilon^{(d)}_{tn}$ and the singular values, $s_{r_\pre}, \varsigma_{r_\post}$. 
%
As such, we employ the heuristic variant in our case studies presented in Section~\ref{sec:empirics}. 

\input{content/SC_case_studies}

















==> content/lit_comparisons.tex <==
\section{Comparison with the Synthetic Controls Literature}\label{sec:causal_param_comparison}
%
The goal of this section is to better contextualize our assumptions and results within the SC literature, by doing a detailed comparison with some representative works.
%

\vspace{2mm}
%
\noindent
%
{\em Causal parameter in SC: treatment effect on the treated. } 
%
For any $(n,d)$ pair, let 
$
\barY_n^{(d)} = \frac{1}{T_1} \sum_{t \in \Tc_\post} Y^{(d)}_{tn}. 
$
%
In addition, let $ \tau_n^{(d_1, d_2)} = \barY^{(d_1)}_n - \barY^{(d_2)}_n$ denote the (relative) treatment effect between interventions $d_1$ and $d_2$ for unit $n$, averaged over the post-intervention period. 
%
The most closely related causal parameter in the SC literature to our work is $\tau_n^{(d,0)}$ for $n \in \Ic^{(d)}$ and $d \neq 0$.
% 
This is referred to as the unit specific treatment effect on the treated, averaged over the post-intervention period. 
% 
Recall $\barY^{(d)}_n$ is observed for $n \in \Ic^{(d)}$.
%
As such, the goal in these works is to estimate the counterfactual potential outcomes $\barY^{(0)}_n$ for $n \notin \Ic^{(0)}$, i.e., what would have happened to a ``treated'' unit $n$ had it remained under control.
%
The quantity $\barY^{(0)}_n$ is closely related to $\theta^{(0)}_n$; the slight difference is that $\theta^{(0)}_n = \Ex[ \barY^{(0)}_n | \{u^{(0)}_t, v_n: t \in \Tc_\post \}]$, where the expectation is taken with respect to the mean zero residual term and conditioned on the latent factors. 
%
Many of the works listed below {\em implicitly} condition on either the latent factors or directly on the observations $Y_{tn}$, if a factor model is not assumed. 

%
We re-emphasize the SI framework allows for identification and inference of $\theta^{(d)}_n$ for $d \neq 0$ and all $n \in [N]$, which these previous works do not consider. 
%
This enables some of the key applications we study, such as synthetic A/B testing described in Section \ref{sec:empirics}.

\vspace{2mm}
%
\noindent
%
{\em Representative works. } 
%
Arguably, $\tau_n^{(d,0)}$ is the most common casual parameter considered in the SC literature, e.g., see  
\cite{Hsiao12, imbens16, athey1, LiBell17, xu_2017, Li18, bai2020matrix, Kwok20, chernozhukov2020practical, fernandezval2020lowrank}. 
%
We restrict our attention to four recent works, \cite{bai2020matrix}, \cite{chernozhukov2020practical}, \cite{ark}, and \cite{agarwal2020robustness} as they highlight some of the primary points of comparison of SI with the SC literature.
%
Again, given the vastness of the literature, we underscore that these comparisons are by no means exhaustive.

%\footnote{A related causal parameter considered in many of these works is the time specific treatment effect on the treated, averaged over all treated units. 
%%%
%%This reduces to estimating $\barY^{(0)}_t = (N-\numdonorscontrol)^{-1}\sum_{n \notin \Ic^{(0)}} Y^{(0)}_{tn}$ for a particular $t > T_0$. 
%%%
%%Estimating this quantity is quite similar to estimating $\barY^{(0)}_n$. 
%%%
%%In particular, we can estimate $\barY^{(0)}_t$ by simply transposing the observations and then running the same estimator used to estimate $\barY^{(0)}_n$.}  
% 
\begin{remark}[Related causal parameter]
A related causal parameter considered in many of these works is the time specific treatment effect on the treated, averaged over all treated units. 
%
This reduces to estimating $\barY^{(0)}_t = (N-\numdonorscontrol)^{-1}\sum_{n \notin \Ic^{(0)}} Y^{(0)}_{tn}$ for a particular $t > T_0$. 
%
Estimating this quantity is quite similar to estimating $\barY^{(0)}_n$. 
%
In particular, we can estimate $\barY^{(0)}_t$ by simply transposing the observations and then running the same estimator used to estimate $\barY^{(0)}_n$.
\end{remark}

\subsection{Comparison with \cite{chernozhukov2020practical}}\label{sec:chero_comparison}
%
\noindent{\em Overview of assumptions. }
%
There are two key assumptions made in \cite{chernozhukov2020practical}.
%
First, the authors assume the existence of $w^{(n, 0)} \in \Rb^{\numdonorscontrol}$ such that for all time $t$ and conditioned on any sampling of $\{Y^{(0)}_{tj}: j \in \Ic^{(0)} \}$, 
%
\begin{align}\label{eq:cherno_form}
Y^{(0)}_{tn} = \sum_{j \in \Ic^{(0)}} w^{(n, 0)}_j Y^{(0)}_{tj} + \varepsilon_{tn},
\end{align}
%
where $\Ex[\varepsilon_{tn}] = 0$ and $\Ex[\varepsilon_{tn} Y^{(0)}_{tj}] = 0$.
%
We note that the conditioning on $\{Y^{(0)}_{tj}: j \in \Ic^{(0)} \}$ is implicit in \cite{chernozhukov2020practical}.
%
Second, they assume the existence of an oracle estimator for $w^{(n, 0)}$, denoted as $\hw^{(n, 0)}$, such that $\|w^{(n, 0)} -  \hw^{(n, 0)}\|_2 = o(1)$.
%

The two most common restrictions placed on $w^{(n, 0)}$, for which there exist estimators with formal performance guarantees, include
%
(i) $w^{(n, 0)}$ is convex, i.e., $\sum_{j \in \Ic^{(0)}} w_j^{(n, 0)} = 1$ and $w_j^{(n, 0)} \ge 0$, cf. \cite{abadie1, abadie2, imbens16}; 
%
(ii) $w^{(n, 0)}$ is approximately sparse, i.e., $\|w^{(n, 0)}\|_1 = O(1)$, which is a relatively weaker assumption, cf. \cite{raskutti11, chernozhukov2020exact}.
%
Under these assumptions, the authors provide a flexible and practical t-test based inference procedure to estimate $\barY^{(0)}_n$, which utilizes the oracle estimator $\hw^{(n, 0)}$.
%
We compare these assumptions with the SI framework.

\vspace{2mm}
%
\noindent{\em Functional form in \eqref{eq:cherno_form}. }
% 
Note that under Assumption \ref{assumption:form}, we can equivalently write Assumption \ref{assumption:linear} as follows: 
%
\begin{align}\label{eq:linear_span_expectation_new}
\Ex[Y^{(d)}_{tn}] = \sum_{j \in \Ic^{(d)}} w^{(n,d)}_j   \Ex[Y^{(d)}_{tj}] \quad \text{for all} \ d.  
\end{align}
%
Compared to \eqref{eq:cherno_form} and for $d=0$, we operate under a weaker functional form assumption as given in \eqref{eq:linear_span_expectation_new}. 
%
To see this, simply take expectations on both sides of \eqref{eq:cherno_form} with respect to $\varepsilon_{tn}$, which implies  \eqref{eq:linear_span_expectation_new}.
%
That is, we do not require the linear relationship $w^{(n, 0)}_j$ to hold between the {\em noisy} potential outcomes $Y^{(0)}_{tn}$ and  $\{Y^{(0)}_{tj}: j \in \Ic^{(0)} \}$. 
%
Rather, we make the weaker assumption that the relationship only holds between the {\em expected} potential outcomes.


\vspace{2mm}
%
\noindent{\em Restrictions on $w^{(n, 0)}$. }
% %
% Another key assumption made is regarding the restrictions placed on $w^{(n, 0)}$. 
%
As discussed, theoretical guarantees in previous works require $w^{(n, 0)}$ to be approximately sparse, or even more stringently, convex.
%
Further, the estimators used to learn $w^{(n, 0)}$ require {\em explicit knowledge} of the restriction placed on $w^{(n, 0)}$. 
%
For example, if $w^{(n, 0)}$ is assumed to be convex, then  convex regression is used; if $w^{(n, 0)}$ is assumed to be approximately sparse, then a $\ell_1$-norm regularizer is used.
%
In comparison, the estimator we propose to learn $w^{(n,0)}$ in \eqref{eq:pcr} does not impose any such restriction on $w^{(n,0)}$, even in the high-dimensional setting where $\numdonorscontrol > \max\{T_0, T_1\}$.
%
Indeed, Lemma \ref{lemma:param_est} establishes that our estimator consistently learns the {\em unique} minimum $\ell_2$-norm $w^{(n,d)}$, denoted as $\tw^{(n,d)}$.   
%
% Further, our consistency and asymptotic normality results {\em implicitly} scale with the $\ell_1$- and $\ell_2$-norm of $\tw^{(n,d)}$. In particular, the error in our consistency result of Theorem \ref{thm:consistency} implicitly scales with $\|\tw^{(n,d)}\|_1$ and the variance in our asymptotic normality result of Theorem \ref{thm:normality} implicitly scales with $\|\tw^{(n,d)}\|_2$.
%

%
We do, however, assume that there exists a latent factor model between the potential outcomes (Assumption \ref{assumption:form}); such an assumption is not made in \cite{chernozhukov2020practical}. 
%
To overcome high-dimensionality, where $w^{(n, d)}$ is not uniquely specified, the estimator in \eqref{eq:pcr} directly exploits the low-rank structure induced by this factor model in Assumption \ref{assumption:form}. 
%

\subsection{Comparison with \cite{bai2020matrix}}\label{sec:bai_comparison}
%
\noindent{\em Overview of assumptions. }
%
In \cite{bai2020matrix}, they consider the following factor model:
%
\begin{align}\label{bai_form}
    Y^{(0)}_{tn} &= \langle x_{tn}, \beta \rangle + \langle F_t, \Lambda_n \rangle + \varepsilon_{tn}
    \\ Y^{(d)}_{tn} &= \alpha^{(d)}_{tn} + Y^{(0)}_{tn}, \ \text{for} \ d \neq 0.
\end{align}
%
Here, $\Lambda_n \in \Rb^{r_1}$ is a unit $n$ specific latent factor and $F_t \in \Rb^{r_1}$ is a time $t$ specific latent factor associated with intervention $d = 0$ (control);  
%
$x_{tn} \in \Rb^k$ is a vector of {\em observed covariates}; and $\beta \in \Rb^k$ is a latent factor acting on $x_{tn}$, which crucially is invariant across $(t,n)$.
%
The authors make appropriate assumptions on the factor loadings $\boldsymbol{\Lambda} = [\Lambda_n] \in \Rb^{r_1 \times N}$  and $\boldsymbol{F} = [F_t] \in \Rb^{r_1 \times T}$, and on the residual term $\varepsilon_{tn}$.
%
See Assumptions A to D in \cite{bai2020matrix} for details. 
%
In essence, these assumptions require 
%
(i) $\boldsymbol{\Lambda}, \boldsymbol{F}$ to satisfy an incoherence-like condition, which implies a bounded operator norm (e.g., $\Ex[\|\boldsymbol{F}\|^4_{\txtop}], \|\boldsymbol{\Lambda}\|_{\txtop} \le M$, where $M$ does not scale with $\numdonorscontrol, T$); 
%
(ii) each of the $r$ singular vectors of $\boldsymbol{\Lambda}, \boldsymbol{F}$ are identifiable (e.g., the non-zero singular values of $\boldsymbol{\Lambda}, \boldsymbol{F}$ are distinct);
%
(iii) $\varepsilon_{tn}$ across $(t,n)$ have sufficiently light tails (e.g., $\Ex[|\varepsilon_{tn}|^8] < M$) and are weakly correlated. 

%
Further, the authors propose an estimator composed of the following main steps: 
%
(i) estimate $\hbeta$ using the observations $\{Y_{tn}, x_{tn}\}$ across $(t,n)$; 
%
(ii) estimate $\widehat{\boldsymbol{\Lambda}}, \widehat{\boldsymbol{F}}$ using the residuals of $\{Y_{tn} - x_{tn}\hbeta\}$; 
%
(iii) estimate $\barY^{(0)}_n$ using $\{x_{tn}, \hbeta, \widehat{\boldsymbol{\Lambda}}, \widehat{\boldsymbol{F}}\}$.
%
Below, we compare their primary assumptions with that of the SI framework.

\vspace{2mm}
\noindent{\em Factor model in \eqref{bai_form}. }
%
First, we compare the factor model assumed in \eqref{bai_form} with that in \eqref{eq:form.0} of Assumption \ref{assumption:form}.
%
Under \eqref{bai_form}, if we further assume that $\langle x_{tn}, \beta \rangle$ admits a latent factorization given by $\langle x_{tn}, \beta \rangle = \langle \tilde{x}_{t}, \tilde{x}_{n}  \rangle$ with $\tilde{x}_{t}, \tilde{x}_{n} \in \Rb^{k_1}$, 
%
then we can write \eqref{bai_form} as a special case of \eqref{eq:form.0}. 
%
To see this, let $d=0$ and define $u^{(0)}_t, v_n \in \Rb^{r}$ in \eqref{eq:form.0} as
%
\begin{align}\label{eq:bai_LFM_SI}
%
u^{(0)}_t = (F_t, \tilde{x}_{t}), \ v_n = (\Lambda_n, \tilde{x}_{n}),
%
\end{align}
where $r=r_1 + k_1$. 
%
We stress that we do not require access to $\tilde{x}_{t}$ or $\tilde{x}_{n}$ to express 
 the model in \cite{bai2020matrix} as an instance of \eqref{eq:form.0}; 
 instead, we require that such a factorization of $\langle x_{tn}, \beta \rangle$ {\em implicitly} exists. 
 %
However, if one does not assume such a latent factorization, then first learning $\beta$ using observed covariates and then estimating $\bLambda, \bF$ via the residuals, is likely necessary. 
%
In Appendix \ref{sec:covariates}, we show how to incorporate covariates in SI. 


%
In addition, if one wants to estimate $\{\theta^{(d)}_n: d \neq 0\}$ in the SI framework (which we underscore is not considered in the SC literature), we require the added assumption that $\alpha^{(d)}_n$ factorizes into a (time, intervention) specific and unit specific latent factor, i.e., 
%
\begin{align}\label{eq:additional_assumption_theta_tnd}
%
\alpha^{(d)}_{tn} = \langle \tilde{\alpha}^{(d)}_{t}, \tilde{\alpha}_{n} \rangle,
%
\end{align}
where $\tilde{\alpha}^{(d)}_{t}, \tilde{\alpha}_{n} \in \Rb^{r_2}$.
%
Then, for $d \neq 0$, we can define $u^{(d)}_t, v_n \in \Rb^{r}$ in \eqref{eq:form.0} as 
%
\begin{align}\label{eq:SI_LFM_additional}
u^{(d)}_t = (F_t, \tilde{x}_{t}, \tilde{\alpha}^{(d)}_{t}), \ v_n = (\Lambda_n, \tilde{x}_{n}, \tilde{\alpha}_{n}),
\end{align}
where $r = r_1 + r_2 + k_1$.
%\footnote{
%%
%In the SC literature, a closely related factor model is  
%$Y^{(0)}_{tn} = \langle \beta_t, x_n \rangle + \langle F_t, \Lambda_n \rangle + \varepsilon_{tn}$ and 
%$Y^{(d)}_{tn} = \alpha^{(d)}_{tn} + Y^{(0)}_{tn}$ for $d \neq 0$, 
%cf. \cite{abadie1, abadie2}. 
%%
%Here, $\beta_t \in \Rb^k$ is a latent factor, $x_n \in \Rb^k$ is an observed unit specific covariate, and $F_t, \Lambda_n \in \Rb^{r_1}$ and $\alpha^{(d)}_{tn} \in \Rb$ are defined as in \eqref{eq:bai_LFM_SI}. 
%%
%As such, similar to \eqref{eq:bai_LFM_SI}, we can write this factor model as a special case of \eqref{eq:form.0},
%where 
%$u^{(0)}_t = (\beta_t, F_t)$ and $\ v_n = (x_n, \Lambda_n)$.
%Again, if one wants to estimate $\theta^{(d)}_{tn}$, then we need to assume an additional factorization of $\alpha^{(d)}_{tn}$, just as in \eqref{eq:additional_assumption_theta_tnd} and \eqref{eq:SI_LFM_additional}.
%}
%
% As before, we do not require observing $\tilde{\alpha}^{(d)}_{t}$ or $\tilde{\alpha}_{n}$, but rather that such a factorization of $\alpha^{(d)}_{tn}$ implicitly exists.
%% In summary, the observed covariates can always be grouped into the associated latent factors. 

\begin{remark}[Closely related factor model]
In the SC literature, a closely related factor model is  
$Y^{(0)}_{tn} = \langle \beta_t, x_n \rangle + \langle F_t, \Lambda_n \rangle + \varepsilon_{tn}$ and 
$Y^{(d)}_{tn} = \alpha^{(d)}_{tn} + Y^{(0)}_{tn}$ for $d \neq 0$, 
cf. \cite{abadie1, abadie2}. 
%
Here, $\beta_t \in \Rb^k$ is a latent factor, $x_n \in \Rb^k$ is an observed unit specific covariate, and $F_t, \Lambda_n \in \Rb^{r_1}$ and $\alpha^{(d)}_{tn} \in \Rb$ are defined as in \eqref{eq:bai_LFM_SI}. 
%
As such, similar to \eqref{eq:bai_LFM_SI}, we can write this factor model as a special case of \eqref{eq:form.0},
where 
$u^{(0)}_t = (\beta_t, F_t)$ and $\ v_n = (x_n, \Lambda_n)$.
Again, if one wants to estimate $\theta^{(d)}_{tn}$, then we need to assume an additional factorization of $\alpha^{(d)}_{tn}$, just as in \eqref{eq:additional_assumption_theta_tnd} and \eqref{eq:SI_LFM_additional}. 
\end{remark} 


\vspace{2mm}
\noindent{\em Assumption on $\boldsymbol{\Lambda}, \boldsymbol{F}$. }
%
Since our ultimate goal is to estimate $\theta^{(d)}_{n}$, it is not necessary to accurately estimate either of the latent factor loadings $(\boldsymbol{\Lambda}, \boldsymbol{F})$. 
%
In fact, our proposed estimator in Section \ref{sec:algo}  explicitly circumvents estimating these two quantities.
%
In comparison, \cite{bai2020matrix} establish their theoretical guarantees by requiring explicit bounds on the estimation qualities of $(\boldsymbol{\Lambda}, \boldsymbol{F})$, which naturally require making more stringent assumptions on the latent factor loadings.
%
% for example, they require each singular vector of $(\boldsymbol{\Lambda}, \boldsymbol{F})$ to be identifiable. 
%

% ADDITIONAL DISCUSSION POINTS 
\subsection{Comparison with \cite{ark} and \cite{agarwal2020robustness}}\label{sec:approx_low_rank_comparison}
%
We compare with these recent works together as they both consider approximately low-rank factor models for the expected potential outcomes, a generalization of what we do.

\vspace{2mm}
%
\noindent
%
{\em Comparison with \cite{ark}.}
%
They consider a binary intervention model:
%
\begin{align}
    \bY^{(0)} &= \bL + \bE,
    \\ \bY^{(1)} &= \bY^{(0)} + \bA,
\end{align}
%
where
%
$\bY^{(0)} = [Y^{(0)}_{tn}] \in \Rb^{T \times N}$ is the matrix of potential outcomes under control; 
$\bL = [L_{tn}] \in \Rb^{T \times N}$ encodes the latent factor model under control (in our notation, $L_{tn} = \langle u^{(0)}_{t}, v_n \rangle$);
$\bE = [\varepsilon_{tn}] \in \Rb^{T \times N}$ encodes the mean zero residuals;
$\bY^{(1)} = [Y^{(1)}_{tn}] \in \Rb^{T \times N}$ is the matrix of potential outcomes under $d=1$; 
and $\bA = [\alpha_{tn}] \in \Rb^{T \times N}$ encodes the treatment effect. 
%
The authors propose the ``synthetic difference-in-differences'' estimator for
%
$\frac{1}{T_1(N - \numdonorscontrol)} \sum_{t \in \Tc_\post} \sum_{n \notin \Ic^{(0)}}\alpha_{tn} | \bL$, 
and establish rigorous asymptotic normality results.


If we continue to restrict our attention to the estimation of counterfactuals under control, then the two primary differences between this work and \cite{ark} are the assumptions made on the
%\cite{ark} differs from our work with respect to 
(i) spectral profile of the factor models and (ii) relationship between the target and donors. 
%
In particular, we consider a low-rank $\bL$ (Assumption \ref{assumption:form}) with a well-balanced spectra (Assumption \ref{assumption:spectra}); the latter effectively assumes a lower bound on the smallest non-zero singular value of $\bL$. 
%
In comparison, \cite{ark} makes a weaker assumption that $\bL$ is {\em approximately} low-rank, i.e., its $\sqrt{\min\{T_0,N_0\}}$-th singular value is sufficiently small (see Assumption 3 of their work).
%
However, as in \cite{abadie2}, they require a convex relationship to hold between the target and donors, while we make the weaker assumption that a linear relationship holds (see the discussion under Assumption~\ref{assumption:linear} for why a linear relationship is directly implied by a low-rank factor model).
%
% Further, we note that in Assumption 4 of \cite{ark}, it is assumed that $\| w^{(n, d)} \|^2_2 = o(\frac{1}{T_1 N_d})$.
% %
% This occurs if the coefficients in $w^{(n, d)}$ are sufficiently disperse.
% %
% However, this would not allow for $w^{(n, d)} = (1, 0, 0, \dots)$, which implies $\| w^{(n, d)} \|^2_2 = 1$.
% %
% This is a case where there is a a unit in $\Ic^{(d)}$ with the exact same latent factor as the target unit, i.e., an exact 1-nearest neighbour exists.
% %
% In comparison our theoretical results imply the SI estimator is consistency, asymptotically normal in such a case. 



\vspace{2mm}
%
\noindent%
{\em Comparison with \cite{agarwal2020robustness}.}
%
They analyze the recently proposed ``robust SC'' (RSC) estimator of \cite{rsc}, which is closely related to our proposed estimator in Section \ref{sec:algo} if restricted to estimating $\theta^{(0)}_n$ for $n \notin \Ic^{(0)}$.
%
The also consider an approximately low-rank $\bL$; specifically, they consider two natural generating processes that induce an approximately low-rank $\bL = [L_{tn}]$: 
%
(i) the spectra of $\bL$ is geometrically decaying (i.e., the $k$-th singular value of $\bL$, denoted as $s_k$, obeys $s_k = s_1 c^{k - 1}$, where $c \in (0, 1)$;
%
(ii) $\bL$ follows a generalized factor model, i.e., $L_{tn} = g(\rho_t, \omega_n)$, where $g(\cdot, \cdot)$ is a latent, H\"{o}lder continuous function, and $\rho_t, \omega_n \in [0, 1]^\ell$ are latent variables associated with time $t$ and unit $n$ (an exact low-rank model is a special case of this where $g$ is bi-linear). 
%
\cite{agarwal2020robustness} establish finite-sample consistency for the RSC estimator with respect to a similar causal parameter as that of $\theta^{(0)}_n$ (see Section 4 of \cite{agarwal2020robustness} for details).
%
However, they do not provide  asymptotic normality results for their target causal parameter. 

\vspace{2mm}
%
\noindent%
{\em Future directions.}
%
An interesting future research direction is to build upon these works to study the trade-offs between the assumptions placed on the latent factor model (e.g., spectral profile), relationship between the target and donors, and subsequent inference guarantees one can establish for various target causal parameters  
%
(e.g., extending the model and estimator of \cite{ark} to estimate $\theta^{(d)}_n$ for any $n \notin \Ic^{(d)}$ and $d \neq 0$).
%
Further, another direction that would be of interest is staggered adoption, where the duration of the pre-intervention period can vary amongst the units, i.e., $T_0$ is specific to each unit.
%
This setup for example was considered in \cite{athey1}.


% \subsection{Statistical Guarantees}\label{sec:stat_gaurantees_comparison}
% %
% As stated earlier, the works listed at the beginning of Section \ref{sec:causal_param_comparison} use some combination (and/or variation) of the assumptions discussed in Sections \ref{sec:chero_comparison} to \ref{sec:approx_low_rank_comparison} to prove formal statistical guarantees.
% %
% To prove asymptotic normality, the works of \cite{chernozhukov2020practical, bai2020matrix, ark}, make additional assumptions on the relative scalings between $T_0$, $T_1$, $\numdonorscontrol$.
% %
% We also make similar assumptions but with respect to $N_d$, rather than $\numdonorscontrol$, to estimate $\htheta^{(d)}_n$ for $d \neq 0$.
% %
% In particular, \cite{chernozhukov2020practical} requires 
% %
% (i) $T_0, T_1 \to \infty$; 
% %
% (ii) $T_0 / T_1 \to c_0$, where $c_o \in [0, \infty]$. 
% %
% \cite{bai2020matrix} requires
% %
% (i) $T_0, T_1, N \to \infty$; 
% %
% (ii) $\sqrt{N} / \min\{\numdonorscontrol, T_0\} \to 0$; 
% %
% and (iii) $\sqrt{T_0 + T_1} / \min\{\numdonorscontrol, T_0\}$ $\to 0$.
% %
% To estimate $\theta^{(d)}_n$, we require
% %
% (i) $T_0, T_1, \numdonors \to \infty$;  
% %
% (ii) $T_1 / \min\{\numdonors, \sqrt{T_0}\} \to 0$.
% %

% \cite{ark} allows for the additional flexibility that they only require the product $(N-N_0)T_1 \rightarrow \infty$.
% %
% As an implication, $N-N_0$ can be a constant as long as $T_1$ grows; hence, if $N-N_0 = 1$, then this is equivalent to $\theta_n^{(0)}$.
% %
% On the other extreme, they allow for $T_1$ to be fixed as long as $N-N_0$ grows; 
% %
% one can verify that our results hold under this setting by using the estimate
% $\frac{1}{N-N_0}\sum_{n \notin \Ic^{(0)}} \sum_{j \in \Ic^{(0)}} \hw_j^{(n,0)} Y_{tj}$. 
% %
% To establish their results, \cite{ark} assume certain relative scalings between $T_0, T_1, N_0, (N-N_0)$ (see Assumption 2 of \cite{ark}), which require that $T_1 (N - N_0)$ do not grow ``too quickly'' compared to $T_0$ and $N_0$. 
% %
% We note that finding the optimal relative scalings between $T_0$, $T_1$, $\numdonorscontrol$ (or $N_d$) remains interesting future work.



==> content/mod_pcr.tex <==
\section{Asymptotic Normality} \label{sec:mod.pcr}
%
As discussed in Section~\ref{ssec:normality}, we have not formally shown that the $\hw^{(n,d)}$ produced from \eqref{eq:pcr} of the \PCR~variant of \SI~satisfies \eqref{eq:cond.iii} of Theorem~\ref{thm:normality}. 
%
Accordingly, we present a slight modification to the \PCR~variant of the \SI~estimator and show that this strategy obeys our desired condition in \eqref{eq:cond.iii}.

% DESCRIPTION 
\medskip 
\subsection{Description of Estimator}  \label{sec:mod.pcr.algo}
%
We recall the notation set in Section~\ref{sec:algo}. 
%
At a high-level, the modified estimator proceeds in the exact same manner as described in Section~\ref{ssec:method} with one change to \eqref{eq:pcr} of step (i). 


Let $\bYpred^k = \sum_{\ell=1}^k \hs_\ell \hu_\ell \hv_\ell^\top$ denote the rank-$k$-approximation of $\bYpred$.
%
%Assuming $k \ge r_\pre$, 
We then construct a sub-sampled matrix that retains the columns of $\bYpred^k$ within an index set $\Omega \subset \cI^{(d)}$. 
%
We denote the resulting matrix as $\bYpred^{(k,\Omega)} \in \Rb^{T_0 \times |\Omega|}$. 
%
Next, we replace \eqref{eq:pcr} with 
%
\begin{align}
	\hw^{(n,d, \Omega)} = \left( \bYpred^{(k, \Omega)} \right)^\dagger \Ynpre \in \Rb^{|\Omega|}, \label{eq:pcr.variant}
\end{align}
%
where $\dagger$ denotes the pseudoinverse. 
%
In words, $\bYpred^{(k, \Omega)}$ retains the de-noised pre-intervention outcomes associated with a subset of the units in $\Ic^{(d)}$; the target unit is then represented by a linear composition defined over $\hw^{(n,d, \Omega)}$ of these selected units. 
%
The rest of the modified estimator continues as described in steps (ii) and (iii) of Section~\ref{ssec:method} with $\hw^{(n,d, \Omega)}$ defined as in \eqref{eq:pcr.variant} and $\bYpostd^\Omega \in \Rb^{T_1 \times |\Omega|}$ defined as the sub-matrix that retains the columns of $\bYpostd$ within $\Omega$. 

% THEORY
\medskip 
\subsection{Theoretical Implications} 
%
As in Section~\ref{sec:formal}, we consider a single $(n,d)$ pair. 
%
To present the theory associated with our modified estimator, we introduce some notation. 
%
Let $\bV_{\cI^{(d)}} = [v_j: j \in \cI^{(d)}] \in \Rb^{\numdonors \times r}$.
%
We define $\bV_{\cI^{(d)}}^\Omega \in \Rb^{|\Omega| \times r}$ as the sub-sampled matrix that retains the rows of $\bV_{\cI^{(d)}}$ within $\Omega$. 


We reemphasize that our donor set is now defined with respect to $\Omega \subset \cI^{(d)}$. 
%
To adapt the results in Section~\ref{sec:formal} to our new setting, we note that if $\Omega$ is chosen such that $\text{span}\{v_j: j \in \Omega\}$ is an $r_\pre$-dimensional subspace of $\Rb^{\numdonors}$, i.e., $\rank(\bV_{\cI^{(d)}}^\Omega) = r_\pre$, then there exists a $w^{(n,d,\Omega)} \in \Rb^{|\Omega|}$ such that 
%
\begin{align}
	v_n = \bV_{\cI^{(d)}}^\top \cdot w_j^{(n,d)} = \left(\bV_{\cI^{(d)}}^\Omega \right)^\top \cdot w_j^{(n,d,\Omega)}, \label{eq:image.compressed}
\end{align} 
%
where $w^{(n,d)} \in \Rb^{\numdonors}$ is defined as in Assumption~\ref{assumption:linear} (and Theorem~\ref{thm:identification}). 
%
% {\color{red}
% To arrive at \eqref{eq:image.compressed}, observe that $\rank(\bV_{\cI^{(d)}}) = r_\pre$ implies that the rows of $\bV_{\cI^{(d)}}$ are necessarily linearly dependent.
% %
% Hence, there exists a vector $\omega \in \Rb^{\numdonors}$ such that $\omega_j = 0$ for all $j \notin \Omega$ and $\bV_{\cI^{(d)}}^\top \cdot w^{(n,d)} = \bV_{\cI^{(d)}}^\top \cdot \omega$. 
% %
% We then define $w^{(n,d,\Omega)}$ as the subvector of $\omega$ that retains its nonzero entries.}


Intuitively, our modified strategy anchors on the concept that only $r_\pre$ donors are needed to recreate our target unit $n$ since $\bV_{\cI^{(d)}}$ has rank $r_\pre$; hence, it suffices to use a subset of donors defined over $\Omega$ rather than utilizing all $N_d$ donor units, provided $\Omega$ is chosen such that \eqref{eq:image.compressed} holds. 
%
With this intuition, we are now ready to present the main result of this section. 
%
Below, let $\bMpred = \Ex[\bYpred \mid \mathcal{E}]$ and define $\bMpred^{\Omega} \in \Rb^{T_0 \times |\Omega|}$ as the sub-sampled matrix that retains the columns of $\bMpred$ within $\Omega$. 


% LEMMA 
\begin{lemma} \label{lemma:cond.iii.compressed}
%
Given $(n,d)$, let Assumptions~\ref{assumption:sutva} to \ref{assumption:subspace} hold. 
%
Consider the modified \PCR~variant of \SI~with $\hw^{(n,d,\Omega)}$ and $w^{(n,d,\Omega)}$ defined as in \eqref{eq:pcr.variant} and \eqref{eq:image.compressed}, respectively.
%
Suppose $k$ and $\Omega$ are chosen such that for appropriate constant $C$, we have
%
\begin{itemize}
	\item[(i)] $k = r_\epre = \rank(\bMepred)$, 
	\item[(ii)] $|\Omega| = r_\epre$ with $\rank(\bYepred^{(r_\epre, \Omega)}) = r_\epre$ and $\rank(\bMepred^\Omega) = r_\epre$,
	\item[(iii)] Assumption~\ref{assumption:spectra} holds with respect to $\bMepred^\Omega$ and $s^\Omega_{r_\epre} \ge C \sigma \sqrt{T_0}$,
	\item[(iv)] $N_d < T_0$,
        \item[(v)] $\| w^{(n,d,\Omega)}) \|_2 \ge C r^{-1/2}_\epre$,
        \item[(vi)] $r^2_\epre = o\left( \frac{\min\{T_0,\numdonors, T^{1/4}_0 \numdonors^{1/2}\}}{\sqrt{\log(T_0 \numdonors)}} \right)$,
        \item[(vii)] $T_1 = o\left( \min\left\{ \frac{N_d}{\log(T_0 N_d) r^4_\epre}, \frac{T^{1/2}_0}{r^2_\epre}  \right\} \right)$. 
\end{itemize}
%
Then conditioned on $\cE$ and $\Omega$, we have that 
%
\begin{align} \label{eq:cond.ii_PCR_variant}
    \frac{ r^{3/2}_\epre \sqrt{\log(T_0 \numdonors)}}{\| w^{(n,d,\Omega)}\|_2 \cdot \min\{T_0,\numdonors, T^{1/4}_0 \numdonors^{1/2}\} }  = o(1),
\end{align}
%
and (iii)
%
\begin{align} \label{eq:cond.iii_PCR_variant}
\frac{1}{\sqrt{T_1} \|w^{(n,d,\Omega)}\|_2} \sum_{t \in \Tc_\post}  \left \langle \Ex[Y^\Omega_{t, \Ic^{(d)}}],  \left( \bM^\Omega_{\epre, \Ic^{(d)}} \right)^\dagger  \bM^\Omega_{\epre, \Ic^{(d)}}\left(\hw^{(n,d, \Omega)} - w^{(n,d,\Omega)} \right) \right \rangle &= o_p(1). 
\end{align}
%
where $\Ex[Y^\Omega_{t, \Ic^{(d)}}] = [\Ex[Y_{tjd}]: j \in \Omega] \in \Rb^{r_\epre}$ and $O_p(\cdot)$ is defined with respect to the sequence $\numdonors$. 
%
That is, conditions \eqref{eq:cond.ii} and \eqref{eq:cond.iii} of Theorem \ref{thm:normality} hold for the modified \PCR~variant of \SI.
\end{lemma} 
%
We note that $(\bM^\Omega_{\pre, \Ic^{(d)}})^\dagger  \bM^\Omega_{\pre, \Ic^{(d)}}$ is exactly the projection onto the row space of $\bM^\Omega_{\pre, \Ic^{(d)}}$, analogous to how $\bV_\pre \bV_\pre^\top$ is defined in \eqref{eq:cond.iii}.

Lemma~\ref{lemma:cond.iii.compressed} states that the modified \PCR-based \SI~estimator satisfies the condition \eqref{eq:cond.iii} required in Theorem~\ref{thm:normality} to achieve asymptotic normality. 
%
In particular, it proves a stronger condition as it does not require $T_1$ to be growing.
%
As such, Theorem~\ref{thm:normality} holds for our modified estimator, which enables us to conduct valid inference via the confidence interval \eqref{eq:finite_sample_CI} of Section \ref{sec:algo}. 

% PROOF
\medskip 
\subsection{Proof of Lemma~\ref{lemma:cond.iii.compressed}} 
%
We state the proof of Lemma~\ref{lemma:cond.iii.compressed}, which is an adaptation of the proof of Lemma~\ref{lemma:pcr_aos2} in Appendix~\ref{sec:consistency.1}.
 
\medskip 
\begin{proof} {Proof of Lemma~\ref{lemma:cond.iii.compressed}.}
%
Below we establish \eqref{eq:cond.ii_PCR_variant} and \eqref{eq:cond.iii_PCR_variant} hold.

\begin{itemize}

\item[(a)] {\em Proof of \eqref{eq:cond.ii_PCR_variant}.} 
%
Holds immediately given conditions (v) and (vi) in the lemma statement. 

\item[(b)] {\em Proof of \eqref{eq:cond.iii_PCR_variant}.} 
%
By condition (ii), the rowspaces of both $\bYpred^{(r_\pre, \Omega)}$ and $\bMpred^\Omega$ span all of $\Rb^{r_\pre}$.
%
Hence, the orthogonal projection matrices onto their rowspaces obey 
%
\begin{align}
	\left( \bYpred^{(r_\pre, \Omega)}\right)^\dagger   \bYpred^{(r_\pre, \Omega)} = \left(\bMpred^\Omega \right)^\dagger \bMpred^\Omega = \bI_{r_\pre}, \label{eq:projection.1} 
\end{align}
%
where $\bI_{r_\pre}$ denotes the $r_\pre \times r_\pre$-dimensional identity matrix.  
%
% In turn, we note that, within our context, $\tw^{(n,d)}$ as defined in \eqref{eq:wtilde} is equivalent to $w^{(n,d,\Omega)}$, which yields condition \eqref{eq:cond.iii} of Theorem~\ref{thm:normality} to be equivalent to  
% %
% \begin{align}
% 	\sqrt{T_1} \cdot \text{LHS of \eqref{eq:cond.iii}} &= \frac{\sqrt{r_\pre} \cdot \| \hw^{(n,d,\Omega)} - w^{(n,d,\Omega)} \|_2} {\| w^{(n,d,\Omega)}) \|_2}. \label{eq:cond.iii.compressed} 
% \end{align} 
%
The remainder of this proof is dedicated to bounding $\Delta^{(n,d,\Omega)} = \| \hw^{(n,d,\Omega)} - w^{(n,d,\Omega)} \|_2$ using the proof of Lemma~\ref{lemma:pcr_aos2} in Appendix~\ref{sec:consistency.1} as a guide. 

Using \eqref{eq:projection.1} and the arguments that led to \eqref{eq:thm1.2}, we obtain 
%
\begin{align} 
%
 \| \Delta^{(n,d, \Omega)}  \|_2^2 
& \leq \frac{4}{(\hs^\Omega_{r_\pre})^2} \left( \| \bYpred^{(r_\pre, \Omega)} - \bMpred^\Omega \|_{2,\infty}^2 \cdot \|\tw^{(n,d,\Omega)}\|_1^2
+\langle \bYpred^{(r_\pre, \Omega)} \cdot \Delta^{(n,d, \Omega)}, \varepsilon_{\pre, n} \rangle\right). \label{eq:compressed.1} 
\end{align}
%
where $\hs^\Omega_{k}$ is defined as the $k$-th singular value of $\bYpred^{(r_\pre, \Omega)}$ while $\varepsilon_{\pre,n}$ maintains the same definition as set in Appendix~\ref{sec:proof_consistency}.
%
By construction, it follows that 
%
\begin{align}
	\| \bYpred^{(r_\pre, \Omega)} - \bMpred^\Omega \|_{2,\infty}^2 \le \| \bYpred^{r_\pre} - \bMpred \|_{2,\infty}^2 \label{eq:compressed.2} 
\end{align} 
%
since $\bYpred^{(r_\pre, \Omega)}$ and $\bMpred^\Omega$ are sub-matrices of $\bYpred^{r_\pre}$ and $\bMpred$, respectively. 

Let $s^\Omega_{k}$ denote the $k$-th singular value of $\bMpred^\Omega$. 
%
Further, without loss of generality, suppose $\Omega$ corresponds to the first $r_\pre$ entries of $\cI^{(d)}$. 
%
This allows us to write 
%
\begin{align}
	\bYpred^{(r_\pre, \Omega)} = \bYpred^{r_\pre} \bA,
	\qquad
	\bMpred^\Omega = \bMpred \bA, \label{eq:transformation}
\end{align} 
%
where $\bA = [\bI_{r_\pre}, 0_{r_\pre \times (\numdonors-r_\pre)}]^\top$. 
%
Combining \eqref{eq:transformation} with Lemma~\ref{lemma:weyl}, we have 
%
\begin{align} 
	| \hs^\Omega_{r_\pre} - s^\Omega_{r_\pre} | &\le \| \bYpred^{(r_\pre, \Omega)} - \bMpred^\Omega \|_\txtop 
	\\ &= \| (\bYpred^{r_\pre} - \bMpred ) \cdot \bA \|_\txtop
	\\ &\le \| \bYpred^{r_\pre} - \bMpred  \|_\txtop  &&\because \| \bA \|_\txtop = 1
	\\ &\le \| \bYpred^{r_\pre} - \bYpred \|_\txtop + \| \bYpred - \bMpred \|_\txtop 
	\\ &= \hs_{r_\pre + 1} + \| \bYpred - \bMpred \|_\txtop, \label{eq:s.compressed.1} 
\end{align} 
%
where we recall $\hs_k$ is the $k$-th singular value of $\bYpred$. 
%
Let us define $s_k$ analogously to $\hs_k$ with respect to $\bMpred$.  
%
By condition (i), $s_{r_\pre+1} = 0$ and thus 
%
\begin{align}
	\hs_{r_\pre+1} &= \hs_{r_\pre+1} - s_{r_\pre+1} 
	\\ &\le \| \bYpred - \bMpred \|_\txtop. &&\because \text{Lemma~\ref{lemma:weyl}}  \label{eq:s.compressed.2} 
\end{align} 
%
Applying Assumption \ref{assumption:noise} and Lemma \ref{lemma:subg_matrix} to \eqref{eq:s.compressed.1} and \eqref{eq:s.compressed.2} yields w.p. at least $1-2\exp(-\zeta^2)$, 
%
\begin{align}
	| \hs^\Omega_{r_\pre} - s^\Omega_{r_\pre} | &\le 2 \cdot \| \bYpred - \bMpred \|_\txtop
	\\ &\le C \sigma \left( \sqrt{T_0} + \sqrt{\numdonors} + \zeta \right) \label{eq:s.compressed.3}
\end{align}  
%
for any $\zeta > 0$. 
%
Next, we follow the arguments that led to \eqref{eq:dd.1}.
%
In particular, we plug \eqref{eq:compressed.2} and \eqref{eq:s.compressed.3} into \eqref{eq:compressed.1}, and invoke Lemmas~\ref{lemma:coeff_bound}, \ref{lemma:hsvt}, \ref{lemma:annoying}, and conditions (iii)--(iv) to conclude
%
\begin{align} \label{eq:new.pcr.rate}
	  \Delta^{(n,d, \Omega)}  &= O_p \left( 
	  \frac{r_\pre \sqrt{ \log(T_0 N_d)}  }{ \sqrt{N_d}} 
	  + \frac{1}{T_0^{1/4}} \right). 
\end{align} 
%
Then,
%
\begin{align}
&\frac{1}{\sqrt{T_1} \|w^{(n,d,\Omega)}\|_2} \sum_{t \in \Tc_\post} \left \langle \Ex[Y^\Omega_{t, \Ic^{(d)}}],  \left( \bM^\Omega_{\pre, \Ic^{(d)}} \right)^\dagger  \bM^\Omega_{\pre, \Ic^{(d)}}\left(\hw^{(n,d, \Omega)} - w^{(n,d,\Omega)} \right) \right \rangle,
%
\\ &\quad \le \frac{1}{\sqrt{T_1} \|w^{(n,d,\Omega)}\|_2} \sum_{t \in \Tc_\post} \| \Ex[Y^\Omega_{t, \Ic^{(d)}}] \|_2 \cdot \| \Delta^{(n,d, \Omega)} \|_2,
%
\\ &\quad\le \frac{1}{\sqrt{T_1} \|w^{(n,d,\Omega)}\|_2} \sum_{t \in \Tc_\post} \sqrt{r_\pre} \cdot \| \Delta^{(n,d, \Omega)} \|_2,
%
% \\ &\quad= O_p \left( \frac{1}{\sqrt{T_1} \|w^{(n,d,\Omega)}\|_2} \sum_{t \in \Tc_\post}  \frac{r^{3/2}_\pre \sqrt{ \log(T_0 N_d)}  }{ \sqrt{N_d}} + \frac{\sqrt{r_\pre}}{T_0^{1/4}} \right)
% %
% \\ &\quad= O_p \left( \frac{1}{\sqrt{T_1}} \sum_{t \in \Tc_\post}  \frac{r^{2}_\pre \sqrt{ \log(T_0 N_d)}  }{ \sqrt{N_d}} + \frac{r_\pre}{T_0^{1/4}} \right)
%
\\ &\quad= O_p \left( \frac{ \sqrt{T_1} r^{2}_\pre \sqrt{ \log(T_0 N_d)}  }{ \sqrt{N_d}} + \frac{ \sqrt{T_1} r_\pre}{T_0^{1/4}} \right), 
%
\\ &\quad= o_p(1),
\end{align}
%
where the second to last line follows from \eqref{eq:new.pcr.rate} and condition (v), and the last line follows from condition (vii).
%
\end{itemize}
%
\end{proof} 

% SIMULATIONS
\subsection{Simulations} 
%
We present a simulation to study the coverage properties of the confidence interval in \eqref{eq:finite_sample_CI} based on the modified \PCR-based \SI~estimator described in Section~\ref{sec:mod.pcr.algo}. 

% DGP 
\medskip 
\subsubsection{Data Generating Process} 
%
We vary $T_0 \in \{200, 400, 600, 800, 1000\}$ and choose $r = 5$. 
%
Motivated by our conditions in Lemma~\ref{lemma:cond.iii.compressed}, we choose $N_d = T_0/2$ and $T_1 = \sqrt{T_0}$ for each $T_0$. 

% latent factors 
\medskip
\noindent {\bf Latent Factors.} 
%
As in Section~\ref{sec:sim.dgp}, we generate the latent factors associated with the donor units, $\bV_{\cI^{(d)}} \in \Rb^{N_d \times r}$, by independently sampling its entries from a standard normal. 
%
Then, we sample $w^{(n,d)} \in \Rb^\numdonors$ by drawing its entries from a uniform distribution over $[0,1]$ and normalizing it to have unit norm. 
%
We define the target unit latent factor as $v_n = \bV_{\cI^{(d)}}^\top \cdot w^{(n,d)}$. 

We define the latent factors for  the pre-intervention outcomes under control as $\bU^{(0)}_\pre$, where its entries are i.i.d. samples from a standard normal. 
%
Next, we sample $\bPhi \in \Rb^{T_1 \times r}$ whose entries are i.i.d. draws from a uniform distribution over $[0, 1]$. 
%
We construct the post-intervention latent factors associated with intervention $d$ as $\bU_\post^{(d)} = \bPhi \cdot \left\{ (\bU_\pre^{(0)})^\dagger \bU^{(0)}_\pre \right\}$. 
%
Our causal parameter is defined as $\theta_n^{(d)} = \textsf{average}(\bU_\post^{(d)} \cdot v_n )$.
% = \textsf{average}(\bU_\post^{(d)} \cdot \bV^\top_{\Ic^{(d)}} \cdot w^{(n,d)})$.  

% observations
\medskip
\noindent {\bf Observations.}
%
We define  
(i) $\Ynpre = \bU^{(0)}_\pre \cdot v_n + \varepsilon_{\pre, n}$, 
(ii) $\bYpred =\bU^{(0)}_\pre \cdot \bV^\top_{\cI^{(d)}} + \bE_{\pre, \Ic^{(d)}}$, 
and
(iii) $\bYpostd = \bU^{(d)}_\post \cdot \bV^\top_{\cI^{(d)}} + \bE_{\post, \Ic^{(d)}}$,
%
where the entries of $\left\{\varepsilon_{\pre, n}, \bE_{\pre, \Ic^{(d)}}, \bE_{\post, \Ic^{(d)}}\right\}$ are i.i.d. samples from a standard normal. 

% Results
\medskip 
\subsubsection{Simulation Results} 
%
From  $\{\Ynpre, \bYpred\}$, we learn $\hw^{(n,d, \Omega)}$ via the modified \PCR-based \SI~estimator given in \eqref{eq:pcr.variant}, where $\Omega$ is chosen to index the first $r$ donors of $\cI^{(d)}$; hence, $| \Omega | = r$. 
%
We then define our estimate as $\htheta_n^{(d, \Omega)} = \textsf{average}( \bYpostd^{\Omega} \cdot \hw^{(n,d,\Omega)} )$ and construct its corresponding confidence interval as per \eqref{eq:finite_sample_CI}, i.e., for $\gamma \in (0,1)$, 
%
\begin{align}
	\mathcal{CI}(\gamma) = \left[ \htheta_n^{(d, \Omega)} \pm \frac{z_{\gamma/2} \cdot \widehat{\sigma}^\Omega  \cdot \|\hw^{(n, d, \Omega)}\|_2}{\sqrt{T_1}} \right],
\end{align}
%
where $\hsigma^\Omega = T_0^{-1} \cdot \| \Ynpre - \bYpred^{(r, \Omega)} \cdot \hw^{(n,d,\Omega)} \|_2^2$. 
%
Table~\ref{table:coverage} reports on the empirical coverage probabilities and average interval lengths for $\theta_n^{(d)}$ at each $T_0$ over $50$ trials, where each trial consists of an independent draw of the latent factors and the observations of size $100$; this amounts to $5000$ total simulation repeats per dimension. 
%
As suggested by Lemma~\ref{lemma:cond.iii.compressed}, we observe that our confidence interval consistently achieves close to the nominal targets of $90\%$ and $95\%$ across all values of $T_0$, albeit the interval lengths can be large due to the poorer prediction quality compared to the standard \PCR-based \SI~estimator of \eqref{eq:pcr}. 


\begin{table} [!t]
\centering 
\caption{Coverage results for the modified \PCR-based \SI~estimator across 5000 replications.} 
\begin{tabular}{@{}lcccc@{}}
\toprule
\midrule 
\multirow{2}{*}{Size of $\Tc_\pre$}
& \multicolumn{2}{c}{$90\%$ nominal coverage}   
& \multicolumn{2}{c}{$95\%$ nominal coverage}   
\\ 
\cmidrule(l){2-3} 
\cmidrule(l){4-5} 
& Coverage probability  & Interval length 
& Coverage probability  & Interval length 
\\
\midrule 
$T_0 = 200$   	 
& 0.88	& 15.66
& 0.94	& 18.66	 
\\
\midrule
$T_0 = 400$      	 
& 0.88	& 18.90
& 0.94	& 22.52
\\
\midrule
$T_0 = 600$      	 
& 0.88	& 8.90
& 0.94	& 10.61
\\
\midrule
$T_0 = 800$    	 
& 0.89	& 7.25
& 0.94	& 8.64 
\\
\midrule
$T_0 = 1000$     	 
& 0.90	& 15.58
& 0.95	& 18.57 
\\
\bottomrule
\end{tabular}
\label{table:coverage}
\end{table}

% \begin{table} [!t]
% \centering 
% \caption{Coverage results for the modified \PCR-based \SI~estimator across 5000 replications.} 
% \begin{tabular}{@{}lcccc@{}}
% \toprule
% \midrule 
% \multirow{2}{*}{Size of $\Tc_\pre$}
% & \multicolumn{2}{c}{$90\%$ nominal coverage}   
% & \multicolumn{2}{c}{$95\%$ nominal coverage}   
% \\ 
% \cmidrule(l){2-3} 
% \cmidrule(l){4-5} 
% & Coverage probability  & Interval length 
% & Coverage probability  & Interval length 
% \\
% \midrule 
% $T_0 = 200$   	 
% & 0.895	& 22.518
% & 0.946	& 26.830	 
% \\
% \midrule
% $T_0 = 400$      	 
% & 0.899	& 36.296
% & 0.946	& 43.246
% \\
% \midrule
% $T_0 = 600$      	 
% & 0.902	& 20.519
% & 0.952	& 24.449
% \\
% \midrule
% $T_0 = 800$    	 
% & 0.893	& 20.572
% & 0.947	& 24.511 
% \\
% \midrule
% $T_0 = 1000$     	 
% & 0.895	& 13.348
% & 0.947	& 15.904 
% \\
% \bottomrule
% \end{tabular}
% \label{table:coverage}
% \end{table}


%
%By condition (ii), the orthogonal projection matrices onto the rowspaces of $\bYpred^{(r_\pre, \Omega)}$ and $\bMpred^\Omega$ satisfy 
%\begin{align}
%	\left( \bYpred^{(r_\pre, \Omega)}\right)^\dagger   \bYpred^{(r_\pre, \Omega)} = \left(\bMpred^\Omega \right)^\dagger \bMpred^\Omega = \bI,
%\end{align}
%%
%where $\bI$ denotes the identity matrix.  
%%
%That is, the rowspaces of both $\bYpred^{(r_\pre, \Omega)}$ and $\bMpred^\Omega$ span all of $\Rb^{r_\pre}$.

%\begin{assumption} [Estimation hyper-parameters] \label{assumption:hyperparameters} 
%%
%%
%
%
%%
%We have that $k = r_\epre = \rank(\Ex[\bYepred])$ and $\Omega$ is chosen such that (i) $|\Omega| = r_\epre$ and (ii) $\rank(\bYepred^{(r_\epre, \Omega)}) = r_\epre$. 
%\end{assumption} 


%Before we establish that our modified \PCR-based \SI~estimator satisfies \eqref{eq:cond.iii} of Theorem~\ref{thm:normality}, we state an additional assumption that is analogous to Assumption~\ref{assumption:spectra}. 
%
%\begin{assumption} [Well-balanced spectra of sub-matrix] \label{assumption:spectra.sub} 
%%
%For any $d$, we denote $r_{\epre} = \rank(\Ex[\bYepred  | \cE ])$ and $\{s_1, \dots, s_{r_{\epre}} \}$ as the nonzero singular values of $\Ex[\bYepred | \cE]$. 
%%
%For universal constants $c, c' > 0$, we have $s_1^{-1} s_{r_{\epre}} \geq c$ with $\|\Ex[\bYepred | \cE]\|_F^2 \geq c' \numdonors T_0$.
%%
%\end{assumption} 

%At a high-level, 
%
%the modification is as follows: 
%%
%(i) obtain a rank-$k$-approximation of $\bYpred$ denoted as $\widehat{\Ex}[\bYpred]$;
%(ii) construct a compressed matrix of $\widehat{\Ex}[\bYpred]$ that retains all of its rows but only keeps $r_\pre$ columns while ensuring the rank of the compressed matrix remains at $r_\pre$; 




















































==> content/model.tex <==
\section{Potential Outcomes Tensor Framework}\label{sec:tfm}
%
In this section, we introduce the tensor factor model across potential outcomes and formally define our target causal parameter. 

% TFM 
\subsection{Tensor Factor Model} 
%
We assume the following latent factor model holds.

%
\begin{assumption}[Latent factor model] \label{assumption:form} 
%
For any $(t,n,d)$, we have that 
%
\begin{align} \label{eq:form.0} 
%
Y_{tn}^{(d)} = \langle u^{(d)}_t,  v_n \rangle + \varepsilon^{(d)}_{tn}, 
%
\end{align} 
%
where $u^{(d)}_t \in \Rb^r$ is the latent factor specific to $(t,d)$; 
%
$v_n \in \Rb^r$ is the latent factor specific to $n$;
%
and $\varepsilon^{(d)}_{tn} \in \Rb$ is a mean zero residual term specific to $(t, n, d)$. 
%
\end{assumption} 
%

Assumption \ref{assumption:form} states that the collection of latent factors, denoted as $\cLF = \{ u^{(d)}_t, v_n : (t,n,d) \}$, determines the expected potential outcomes $\Ex[Y_{tn}^{(d)}] = \langle u^{(d)}_t,  v_n \rangle$; here, the expectation is taken with respect to $\varepsilon^{(d)}_{tn}$.
%
We further interpret Assumption \ref{assumption:form} through the lens of tensor factor models below.
%
\begin{definition}[Tensor factor model]\label{def:tfm}
%
{\em The expected potential outcome of $Y^{(d)}_{tn}$ satisfies a tensor factor model if it has the following representation: 
%
\begin{align} \label{eq:tfm}
%
\Ex[Y^{(d)}_{tn}] & = \sum_{\ell=1}^r u_{t \ell} v_{n \ell} \lambda_{d \ell}, 
%
\end{align}
%
where $r$ is the canonical polyadic rank, and
%
$u_{t}, v_{n}, w_{d} \in \Rb^r$ are the latent factors associated with the $t$-th measurement, $n$-th unit, and $d$-th intervention, respectively.
}
%
\end{definition}

The tensor factor model is a natural generalization of the matrix factor model considered in the literature. 
%
Along with assuming latent factorization across units and measurements as is traditionally done in panel data settings, the tensor factor model also assumes latent factorization across interventions.
%
When restricted to intervention $d$, we can re-write the tensor factor model as
%
\begin{align}\label{eq:a.1}
%
\Ex[Y_{tn}^{(d)}] & = \langle u^{(d)}_t,  v_n \rangle
%
\end{align}
%
where $u^{(d)}_t = [u_{t \ell} \lambda_{d \ell}: \ell \in [r]] \in \Rb^r$ 
and $v_n = [v_{n \ell}: \ell \in [r]] \in \Rb^r$. 
%
Indeed, \eqref{eq:a.1} states that the expected potential outcomes should satisfy the traditional matrix factor model separately for each intervention.
%
The critical additional assumption is that $v_n$ remains invariant across interventions. 
%
In this work, we shall require this weaker condition as summarized in Assumption \ref{assumption:form}, which is implied by the tensor factor model. 

% REMARK 
\begin{remark} [Non-linear latent variable models]
%
In Appendix~\ref{sec:nonlinear_lvm}, we show that sufficiently continuous non-linear latent variable models are arbitrarily well-approximated by linear factor models of the form \eqref{eq:form.0} in Assumption \ref{assumption:form} as $N$ and $T$ grow. 
%
\end{remark} 

% CAUSAL PARAMETERS
\subsection{Causal Parameters}\label{sec:causal_param}
%
Given Assumption \ref{assumption:form}, we formally define our causal parameters.
%
For every $(n,d)$ pair, we are interested in estimating
%
\begin{align}\label{eq:target_causal_parameter}
%
\theta^{(d)}_n & = \frac{1}{T_1} \sum_{t \in \Tc_\post} \Ex\left[  Y^{(d)}_{tn} ~\Big|~ \{u^{(d)}_t, v_n: t \in \Tc_\post \} \right],
%
\end{align}
%
which represents the expected potential outcome for unit $n$ under intervention $d$ averaged over the target measurements in $\Tc_\post$, conditioned on the latent factors. 
%
We reemphasize that the expectation is taken over $\varepsilon^{(d)}_{tn}$, as defined in Assumption \ref{assumption:form}.


%We are interested in estimating $\theta^{(d)}_n = |\Tc_\post|^{-1} \sum_{t \in \Tc_{\post}} \Ex[Y^{(d)}_{tn}]$, which represents the expected potential outcome for unit $n$ under intervention $d$ averaged over the target measurements in $\Tc_\post$. 
%%
%In observational settings, we underscore that the potential outcomes $Y^{(d)}_{tn}$ might be correlated with how the entries of $\bY$ are revealed. 
%%
%This serves as an additional challenge in defining an appropriate causal framework to estimate $\theta^{(d)}_n$.





==> content/notations.tex <==
\subsection{Standard Notation}\label{sec:notation}
%
%The columnspace (or range) of $\bA$ is the span of its columns, which we denote as  
%$\Rc(\bA) = \{v \in \Rb^a: v = \bA x, x \in \Rb^b\}$. 
%%
%The rowspace of $\bA$, given by $\Rc(\bA')$, is the span of its rows. 
%%
%Recall that the nullspace of $\bA$ 
%is the set of vectors that are mapped to zero under $\bA$. 
%
For any vector $v \in \Rb^a$, let $\|v\|_p$ denote its 
$\ell_p$-norm. 
%
We define the inner product between vectors $v, x \in \Rb^a$ as 
$\langle v, x \rangle = v^\top x = \sum_{\ell=1}^a v_\ell x_\ell$. 
%
For a matrix $\bA \in \Rb^{a \times b}$, we denote its operator (spectral) and Frobenius norms as $\|\bA\|_{\txtop}$ and $\|\bA\|_F$, respectively.  
%
If $v$ is a random variable, we define its sub-Gaussian (Orlicz) norm as $\|v\|_{\psi_2}$.  
%

Let $f$ and $g$ be two functions defined on the same space. We say that $f(n)$ = $O(g(n))$ if and only if
there exists a positive real number $M$ and a real number $n_0$ such that for all $n \ge n_0, |f (n)| \le M|g(n)|$.
%
Analogously we say:
$f (n) = \Theta(g(n))$ if and only if there exists positive real numbers $m, M$ such that for all $n \ge n_0, \ m|g(n)| \le |f(n)| \le M|g(n)|$;
%
$f (n) = o(g(n))$ if for any $m > 0$, there exists $n_0$ such that for all 
$n \ge n_0, |f(n)| \le m|g(n)|$.

%We adopt the standard notations and definitions for stochastic convergences. 
%
We denote $\xrightarrow{d}$ and $\xrightarrow{p}$ as convergences in distribution and probability, respectively. 
%
%Let $O_p$ and $o_p$, which are probabilistic versions of the deterministic $O$ and $o$ notations. 
%
For any sequence of random vectors $X_n$, we say $X_n = O_p(a_n)$ if for every $\varepsilon>0$, there exists constants $C_\varepsilon$ and $n_\varepsilon$ such that $\Pb( \| X_n \|_2 > C_\varepsilon a_n) < \varepsilon$ for every $n \ge n_\varepsilon$. 
%
%equivalently, we say $(1/a_n) X_n$ is ``uniformly tight'' or ``bounded in probability''.
%
Similarly, $X_n = o_p(a_n)$ if for all $\varepsilon, \varepsilon'> 0$, there exists $n_\varepsilon$ such that $\Pb(\| X_n \|_2 > \varepsilon' a_n) < \varepsilon$ for every $n \ge n_\varepsilon$.
%
Therefore, $X_n = o_p(1) \iff X_n \xrightarrow{p} 0$. 
%
%Additionally, we use the ``plim'' probability limit operator: $\text{plim} \ X_n = a \iff X_n \xrightarrow{p} a$. 
%
We say a sequence of events $\Ec_n$
holds ``with high probability'' (w.h.p.) if $\Pb(\Ec_n) \rightarrow 1$ as $n \rightarrow \infty$, i.e., for any $\varepsilon > 0$, there exists a $n_\varepsilon$ such that for all $n > n_\varepsilon$, $\Pb(\Ec_n) > 1 - \varepsilon$. More generally, a multi-indexed 
sequence of events $\Ec_{n_1,\dots, n_d}$, with indices $n_1,\dots, n_d$ with $d \geq 1$, is said to 
hold w.h.p. if $\Pb(\Ec_{n_1,\dots, n_d}) \rightarrow 1$ as $\min\{n_1,\dots, n_d\} \rightarrow \infty$.
%
%We also use $\Nc(\mu, \sigma^2)$ to denote a normal or Gaussian distribution with mean $\mu$ and variance $\sigma^2$; we call it {\em standard} normal or Gaussian if $\mu = 0$ and $\sigma^2 = 1$.






==> content/proofs_hypo_lems.tex <==


% TYPE I LEMMA
\subsection{Proof of Lemma \ref{lemma:type1.1}} \label{sec:type1_lem}
% \vspace{-5pt}
% To begin, observe that
{\small
$
	\htau = \|(\bI - \Pc_{\hV_\pre}) \bhV_\post\|_F^2 
	= \|(\bI - \Pc_{\hV_\pre}) \bhV_\post - (\bI - \Pc_{V_\pre}) \bhV_\post + (\bI - \Pc_{V_\pre}) \bhV_\post\|_F^2
	= \|(\Pc_{V_\pre} - \Pc_{\hV_\pre}) \bhV_\post + (\bI - \Pc_{V_\pre}) \bhV_\post\|_F^2
	= \|(\Pc_{V_\pre} - \Pc_{\hV_\pre}) \bhV_\post\|_F^2 + \|(\bI - \Pc_{V_\pre}) \bhV_\post\|_F^2
	 + 2 \langle (\Pc_{V_\pre} - \Pc_{\hV_\pre}) \bhV_\post, (\bI - \Pc_{V_\pre}) \bhV_\post \rangle_F. \label{eq:type1.0.new}
$ 
}

Under $H_0$, it follows that $(\bI - \Pc_{V_\pre}) \bV_\post = 0$. 
As a result, 
$
	 \|(\bI - \Pc_{V_\pre}) \bhV_\post\|_F^2 =  \|(\bI - \Pc_{V_\pre}) \Pc_{\hV_\post}\|_F^2
	 = \|(\bI - \Pc_{V_\pre}) \Pc_{\hV_\post} - (\bI - \Pc_{V_\pre}) \Pc_{V_\post} \|_F^2
	 = \|(\bI - \Pc_{V_\pre}) (\Pc_{\hV_\post} - \Pc_{V_\post})\|_F^2. 
$

Applying these two sets of equalities above together completes the proof. 
 
% TYPE II
\subsection{Proof of Lemma \ref{lemma:type2}} \label{sec:type2_lem}
%
Because the columns of $\bhV_\post$ are orthonormal, 
%
$
	r_\post = \|\bhV_\post\|_F^2 = \| \Pc_{\hV_\pre} \bhV_\post\|_F^2 + \|(\bI - \Pc_{\hV_\pre}) \bhV_\post\|_F^2. 
$
%
Therefore, it follows that
%
\begin{align}
	\htau &= \|(\bI - \Pc_{\hV_\pre}) \bhV_\post\|_F^2  
	= r_\post - \| \Pc_{\hV_\pre} \bhV_\post\|_F^2. \label{eq:type2.0_new}
\end{align}
%
Now, consider the second term of the equality above.  
%
{\small
\begin{align} \label{eq.1} 
	&\|\Pc_{\hV_\pre} \bhV_\post\|_F^2 = %
	\|\Pc_{\hV_\pre} \bhV_\post - \Pc_{V_\pre} \bhV_\post + \Pc_{V_\pre} \bhV_\post\|_F^2
	%
	\\ &= \| (\Pc_{\hV_\pre} - \Pc_{V_\pre}) \bhV_\post\|_F^2 + \|\Pc_{V_\pre} \bhV_\post\|_F^2
	%
	+ 2 \langle (\Pc_{\hV_\pre} - \Pc_{V_\pre}) \bhV_\post, \Pc_{V_\pre} \bhV_\post \rangle_F.
	%
	\label{eq:type2.1_new} 
\end{align} 
}
%
Further, analyzing the second term of \eqref{eq:type2.1_new}, we note that 
%
{\small
\begin{align}
	&\|\Pc_{V_\pre} \bhV_\post\|_F^2 = \|\Pc_{V_\pre} \Pc_{\hV_\post}\|_F^2
	%
	= \| \Pc_{V_\pre} \Pc_{\hV_\post} - \Pc_{V_\pre} \Pc_{V_\post} + \Pc_{V_\pre} \Pc_{V_\post}\|_F^2
	%
	\\ &= \| \Pc_{V_\pre} (\Pc_{\hV_\post} - \Pc_{V_\post})\|_F^2 + \|\Pc_{V_\pre} \Pc_{V_\post}\|_F^2 
	%
	+ 2 \langle \Pc_{V_\pre} (\Pc_{\hV_\post} - \Pc_{V_\post}),  \Pc_{V_\pre} \Pc_{V_\post}\rangle_F.
	%
	\label{eq:type2.2_new} 
\end{align}
}
%
Incorporating \eqref{eq:type2.1_new} and \eqref{eq:type2.2_new} into \eqref{eq:type2.0_new}, and recalling $c_1 = \|\Pc_{V_\pre} \Pc_{V_\post}\|_F^2 = \|\bV_\pre \bV'_\pre \bV_\post\|_F^2 $ completes the proof. 



==> content/proofs_hypo_thm.tex <==
%\section{Proof: Subspace Inclusion Hypothesis Test}
%In this section, we prove Theorem \ref{thm:hypo}. 
%
\section{Proof of Theorem \ref{thm:hypo}} 
For ease of notation, we suppress the conditioning on $\Ec$ for the remainder of the proof.
%
We make use of the following notation: for any matrix $\bA$ with orthonormal columns, let $\Pc_A = \bA \bA^\prime$ denote the projection matrix onto the subspace spanned by the columns of $\bA$.
%
Additionally, we follow the notation established in Section \ref{sec:hypothesis.test}. 
%
In particular, we recall $\phi_\pre(a) = \sqrt{T_0} + \sqrt{N_d} + \sqrt{\log(1/a)}$;
%
$\phi_\post(a) = \sqrt{T_1} + \sqrt{N_d} + \sqrt{\log(1/a)}$; 
%
and $s_\ell, \varsigma_\ell$ are the $\ell$-th singular values of $\Ex[\bYpred]$ and $\Ex[\bYpostd]$, respectively. 
%
Finally, we let $C \ge 0$ denote an absolute constant, whose value can change from line to line or even within a line.


\vspace{10pt} \noindent 
%
{\em Type I error. } 
%
We first bound the Type I error, which anchors on Lemma \ref{lemma:type1.1}, stated below. The proof of Lemma \ref{lemma:type1.1} can be found in Appendix \ref{sec:type1_lem}.

\begin{lemma} \label{lemma:type1.1}
	Suppose $H_0$ is true. Then, 
	
	
\begin{align} \label{eq:type1.1} 
	\htau &= \|(\Pc_{V_\epre} - \Pc_{\hV_\epre}) \bhV_\epost\|_F^2 + 
	\|(\bI - \Pc_{V_\epre}) (\Pc_{\hV_\epost} - \Pc_{V_\epost})\|_F^2
	\\ &\quad + 2 \langle (\Pc_{V_\epre} - \Pc_{\hV_\epre}) \bhV_\epost, (\bI - \Pc_{V_\epre}) \bhV_\epost \rangle_F.
\end{align} 
\end{lemma} 

We proceed to bound each term on the right-hand side of \eqref{eq:type1.1} independently. 

\vspace{10pt} \noindent 
{\em Bounding $\|(\Pc_{V_\epre} - \Pc_{\hV_\epre}) \bhV_\epost\|_F^2$. } 
%
By Lemma \ref{lemma:subspace}, we have w.p. at least $1- \alpha_1$, 
%
{\small
\begin{align}  
	\| (\Pc_{\hV_\pre} - \Pc_{V_\pre}) \bhV_\post \|_F^2 
	&\le \| \Pc_{\hV_\pre} - \Pc_{V_\pre}\|_\txtop^2 ~ \|\bhV_\post\|_F^2
	\le \frac{C \sigma^2 r_\post \phi^2_\pre(\alpha_1)}{s^2_{r_\pre}}.  \label{eq:t.1}
\end{align} 
}
%
Note that we have used the fact that $\| \bhV_\post \|_F^2 = r_\post$. 

\vspace{10pt} \noindent 
%
{\em Bounding $\|(\bI - \Pc_{V_\epre}) (\Pc_{\hV_\epost} - \Pc_{V_\epost})\|_F^2$. } 
Observe that $(\bI - \Pc_{V_\pre})$ is a projection matrix, and hence $\|\bI - \Pc_{V_\pre}\|_\txtop \le 1$. 
%
% Next, we apply Lemma \ref{lemma:subspace} to obtain w.p. at least $1-\alpha_2$,
By adapting Lemma \ref{lemma:subspace} for $\bhV_\post, \bV_\post$ in place of $\bhV_\pre, \bV_\pre$, 
we have w.p. at least $1-\alpha_2$
\begin{align} \label{eq:adapt.1} 
    \| \Pc_{\hV_\post} - \Pc_{V_\post}\|_F^2 
    &\le  r_\post \| \Pc_{\hV_\post} - \Pc_{V_\post}\|_\txtop^2 
    \le \frac{C \sigma^2 r_\post \phi^2_\post(\alpha_2)}{\varsigma^2_{r_\post}}.
\end{align} 
%
Note that we have used the following: 
(i) $\| \Pc_{\hV_\post} - \Pc_{V_\post}\|_F =
\| \sin \Theta \|_F$, where $\sin \Theta \in \Rb^{r_\post \times r_\post}$ is a matrix of principal angles between the two projectors (see \cite{ABSIL2006288}), which implies $\rank(\Pc_{\hV_\post} - \Pc_{V_\post}) \le r_\post$;
%
(ii) the standard norm inequality $\| \bA \|_F \le \sqrt{\rank(\bA)} \| \bA \|_\txtop$ for any matrix $\bA$. 
%
Using the result above, we have 
%
{\small
\begin{align}
	\| (\bI - \Pc_{V_\pre}) (\Pc_{\hV_\post} - \Pc_{V_\post})\|_F^2 &\le 
	\|\bI - \Pc_{V_\pre}\|_\txtop^2 ~ \| \Pc_{\hV_\post} - \Pc_{V_\post}\|_F^2
	\le \frac{C \sigma^2 r_\post \phi^2_\post(\alpha_2)}{\varsigma^2_{r_\post}}.  \label{eq:t.2} 
\end{align} 
}

\vspace{5pt} \noindent 
{\em Bounding $\langle (\Pc_{V_\epre} - \Pc_{\hV_\epre}) \bhV_\epost, ~(\bI - \Pc_{V_\epre}) \bhV_\epost \rangle_F$. } 
Using the cyclic property of the trace operator, we have that
{\small
\begin{align}
	 &\langle (\Pc_{\hV_\pre} - \Pc_{V_\pre}) \bhV_\post, ~ (\bI - \Pc_{V_\epre}) \bhV_\post \rangle_F 
	 %
	= \tr \big( \bhV_\post^\prime (\Pc_{\hV_\pre} - \Pc_{V_\pre})  (\bI - \Pc_{V_\epre}) \bhV_\post \big)
	%
	\\&= \tr \big( (\Pc_{\hV_\pre} - \Pc_{V_\pre})  (\bI - \Pc_{V_\epre}) \Pc_{\hV_\post} \big). \label{eq:helper_type_2_trace}
\end{align} 
}
Note that $\Pc_{\hV_\pre} - \Pc_{V_\pre}$ is symmetric, and $\bI - \Pc_{V_\epre}$ and $\Pc_{\hV_\post}$ are both symmetric positive semidefinite (PSD). As a result, 
Lemmas \ref{lemma:subspace} and \ref{lemma:trace.2} yield w.p. at least $1-\alpha_1$ 
\begin{align}
	&\tr \big( (\Pc_{\hV_\pre} - \Pc_{V_\pre})  (\bI - \Pc_{V_\epre}) \Pc_{\hV_\post} \big)
	%
	\le \| \Pc_{\hV_\pre} - \Pc_{V_\pre} \|_\txtop  \tr \big( (\bI - \Pc_{V_\epre}) \Pc_{\hV_\post} \big) 
	%
	\\ &\le \| \Pc_{\hV_\pre} - \Pc_{V_\pre} \|_\txtop  \| \bI - \Pc_{V_\epre} \|_\txtop  \tr \big( \Pc_{\hV_\post} \big) 
	%
	\le \frac{C \sigma r_\post \phi_\pre(\alpha_1)}{s_{r_\pre}}.
	\label{eq:t.3} 
\end{align} 
Again, to arrive at the above inequality, we use $\| \bI - \Pc_{V_\epre}\|_\txtop \le 1$ and $\text{tr}(\Pc_{\hV_\post}) = r_\post$. 

\vspace{10pt} \noindent {\em Collecting terms. } 
Collecting \eqref{eq:t.1}, \eqref{eq:t.2}, and \eqref{eq:t.3} with $\alpha_1 = \alpha_2 = \alpha/2$,  w.p. at least $1-\alpha$, 
\begin{align}
	\htau &\le 
	\frac{C \sigma^2 r_\post \phi^2_\pre(\alpha/2)}{s^2_{r_\pre}}
	+
	\frac{C \sigma^2 r_\post \phi^2_\post(\alpha/2)}{\varsigma^2_{r_\post}}
	+ 
	\frac{C \sigma r_\post \phi_\pre(\alpha/2)}{s_{r_\pre}}. 
\end{align}
Defining the upper bound as $\tau(\alpha)$ completes the bound on the Type I error. 

%*********
% TYPE II 
%*********
\vspace{10pt} \noindent
{\em Type II error. }
Next, we bound the Type II error. 
We will leverage Lemma \ref{lemma:type2}, the proof of which can be found in Appendix \ref{sec:type2_lem}. 

\begin{lemma} \label{lemma:type2}
The following equality holds: $\htau = r_\epost - c_1 - c_2$, where 
%
{\small
\begin{align} 
    c_1 &= \|\bV_\pre \bV'_\pre \bV_\post\|_F^2
    %
    \\ c_2 &= \|(\Pc_{\hV_\epre} - \Pc_{V_\epre}) \bhV_\epost\|_F^2
    + \|\Pc_{V_\epre} (\Pc_{\hV_\epost} - \Pc_{V_\epost})\|_F^2
    %
    \\ &\quad + 2 \langle (\Pc_{\hV_\epre} - \Pc_{V_\epre}) \bhV_\epost, \Pc_{V_\epre} \bhV_\epost \rangle_F
    %
    + 2 \langle \Pc_{V_\epre} (\Pc_{\hV_\epost} - \Pc_{V_\epost}),  \Pc_{V_\epre} \Pc_{V_\epost} \rangle_F. \label{eq:type2.1} 
\end{align} 
}
\end{lemma} 
%
We proceed to bound each term on the right hand side of \eqref{eq:type2.1} separately. 

% term 1
\vspace{10pt} \noindent 
{\em Bounding $\|(\Pc_{\hV_\epre} - \Pc_{V_\epre}) \bhV_\epost\|_F^2$. } 
From \eqref{eq:t.1}, we have that w.p. at least $1-\alpha_1$, 
\begin{align}  \label{eq:t.5}
	\|(\Pc_{\hV_\pre} - \Pc_{V_\pre}) \bhV_\post \|_F^2 
	&\le \frac{C \sigma^2 r_\post \phi^2_\pre(\alpha_1)}{s^2_{r_\pre}}. 
\end{align} 

% term 2
\vspace{5pt} \noindent 
{\em Bounding $\|\Pc_{V_\epre} (\Pc_{\hV_\epost} - \Pc_{V_\epost})\|_F^2$. } 
%
Using the inequality $\|\bA \bB \|_F \le \|\bA \|_\txtop \|\bB \|_F$ for any two matrices $\bA$ and $\bB$, as well as the bound in  \eqref{eq:adapt.1}, we have w.p. at least $1-\alpha_2$, 
%
\begin{align}  \label{eq:t.6}
	\| \Pc_{V_\pre} (\Pc_{\hV_\post} - \Pc_{V_\post}) \|_F^2 
	&\le \frac{C \sigma^2 r_\post \phi^2_\post(\alpha_2)}{\varsigma^2_{r_\post}}.
\end{align}

% term 3
\vspace{10pt} \noindent 
{\em Bounding $\langle (\Pc_{\hV_\epre} - \Pc_{V_\epre}) \bhV_\epost, \Pc_{V_\epre} \bhV_\epost \rangle_F$. } 
Using an identical argument used to create the bounds in \eqref{eq:helper_type_2_trace} and \eqref{eq:t.3}, but replacing $\bI - \Pc_{V_\pre}$ with $\Pc_{V_\pre}$, we obtain w.p. at least $1-\alpha_1$
\begin{align} \label{eq:t.7}
	 \langle (\Pc_{\hV_\pre} - \Pc_{V_\pre}) \bhV_\post, \Pc_{V_\pre} \bhV_\post \rangle_F 
	& \le  \frac{C \sigma r_\post \phi_\pre(\alpha_1)}{s_{r_\pre}}.
\end{align} 


% term 4
\vspace{5pt} \noindent 
{\em Bounding $\langle \Pc_{V_\epre} (\Pc_{\hV_\epost} - \Pc_{V_\epost}),  \Pc_{V_\epre} \Pc_{V_\epost} \rangle_F$. }
%
Like in the argument to produce the bound in \eqref{eq:t.3}, we use Lemmas \ref{lemma:subspace} and \ref{lemma:trace.2} to get that w.p. at least $1-\alpha_2$, 
%
{\small
\begin{align}
&\langle \Pc_{V_\pre} (\Pc_{\hV_\post} - \Pc_{V_\post}), \Pc_{V_\pre} \Pc_{V_\post} \rangle_F
 = \tr \big( (\Pc_{\hV_\post} - \Pc_{V_\post}) \Pc_{V_\pre} \Pc_{V_\pre} \Pc_{V_\post} \big) 
\\&= \tr \big( (\Pc_{\hV_\post} - \Pc_{V_\post}) \Pc_{V_\pre} \Pc_{V_\post} \big)
\le \| \Pc_{\hV_\post} - \Pc_{V_\post} \|_\txtop ~ \|\Pc_{V_\pre}\|_\txtop  \tr \big( \Pc_{V_\post} \big) 
\le \frac{C \sigma r_\post \phi_\post(\alpha_2)}{\varsigma_{r_\post}}. \label{eq:t.8} 
\end{align} 
}

% combining
\noindent {\em Collecting terms. }
Combining \eqref{eq:t.5}, \eqref{eq:t.6}, \eqref{eq:t.7}, \eqref{eq:t.8} with $\alpha_1 = \alpha_2 = \alpha/2$, and using the definition of $\tau(\alpha)$, we have that w.p. at least $1-\alpha$,
% \begin{align}\label{eq:c_prime_bound}
% 	c_2 &\le \tau(\alpha) + \frac{C \sigma r_\post \phi_\post(\alpha/2)}{\varsigma_{r_\post}}.
% \end{align} 
$$
	c_2 \le \tau(\alpha) + \frac{C \sigma r_\post \phi_\post(\alpha/2)}{\varsigma_{r_\post}}.
$$
%
Hence, along with using Lemma \ref{lemma:type2}, it follows that w.p. at least $1-\alpha$,
\begin{align}\label{eq:unonditional_type_2_bound}
	\htau &\ge r_\post - c_1 - \tau(\alpha) - \frac{C \sigma r_\post \phi_\post(\alpha/2)}{\varsigma_{r_\post}}. 
\end{align} 
%
Now, suppose $r_\post$ satisfies \eqref{eq:type2_cond}, which implies that $H_1$ must hold. 
%
Then, \eqref{eq:unonditional_type_2_bound} and \eqref{eq:type2_cond} together imply  $\Pb(\htau > \tau(\alpha) | H_1) \ge 1 - \alpha$. 
This completes the proof. 


\subsection{Proof of Corollary \ref{cor:hypo}}
%
We utilize Lemmas  \ref{lemma:subg_matrix_gaussian} and \ref{lem:wedin_gaussian}, which are sharp versions of Lemmas \ref{lemma:subg_matrix} and \ref{lemma:subspace}.%, respectively. 
%

\begin{lemma} [Gaussian Matrices: Theorem 7.3.1 of \cite{vershynin2018high}] \label{lemma:subg_matrix_gaussian}
%
Let the setup of Lemma \ref{lemma:subg_matrix} hold.
%
Assume $A_{ij}$ are Gaussian r.v.s with variance $\sigma^2$. Then for any $t > 0$,  
$
    \| \bA \|_{\eop} \le \sigma (\sqrt{m} + \sqrt{n} + t)
$
w.p. at least $1-2\exp(-t^2)$. 
\end{lemma} 

\begin{lemma}\label{lem:wedin_gaussian}
Let the setup of Lemma \ref{lemma:subspace} hold.
%
Further, assume $\varepsilon_{tn}$ are Gaussian r.v.s with variance $\sigma^2$. 
%
Then for any $\alpha \in (0,1)$, we have w.p. at least $1-\alpha$, 
%
\begin{align}
        \| \Pc_{\hV_\epre} - \Pc_{V_\epre} \|_\eop 
        \le \frac{2 \sigma \phi_\epre(\alpha)}{s_{r_\epre}},
        ~~
          \| \Pc_{\hV_\epost} - \Pc_{V_\epost} \|_\eop 
        \le \frac{2 \sigma \phi_\epost(\alpha)}{\varsigma_{r_\epost}}. 
    \end{align}
    %w.p. at least $1-\alpha$. 
\end{lemma}

\begin{proof}
%
The proof is identical to that of Lemma \ref{lemma:subspace} except $\| \bY_{\pre, \Ic^{(d)}} - \Ex[\bY_{\pre, \Ic^{(d)}}] \|_\txtop$ is now bounded above using Lemma \ref{lemma:subg_matrix_gaussian}. 
\end{proof}
%
The remainder of the proof of Corollary \ref{cor:hypo} is identical to that of Theorem \ref{thm:hypo}.











==> content/simulation_details.tex <==
\section{Simulation Details} \label{sec:simulation_details}
%
In this section, we present the details of our simulations in Section~\ref{sec:simulations}. 

% CONSISTENCY
\subsection{Consistency}
%
Below, we provide details for our consistency simulation in Section~\ref{sec:sim_consistency}. 

\subsubsection{Generative Model for Synthetic Data} \label{ssec:empirics_consistency_model} 
%
We let $N_d = | \Ic^{(d)}| = 200$ and $r = 15$, where $r$ is defined in Assumption \ref{assumption:form}. 
%
We define the latent unit factors associated with $\Ic^{(d)}$ as $\bV_{\Ic^{(d)}} \in \Rb^{N_d \times r}$ (refer to \eqref{eq:form.0}), where its entries are independently sampled from a standard normal distribution. 

\vspace{10pt} 
\noindent 
{\em Pre-intervention data.} We choose $T_0 = 200$ and $r_\pre = 10$. 
%
We define the latent pre-intervention time factors under control ($d=0$) as $\bU_\pre \in \Rb^{T_0 \times r}$, which is sampled as follows: 
%
(i) let $\bA \in \Rb^{T_0 \times r_\pre}$, where its entries are independently sampled from a standard normal; 
%
(ii) let $\bQ \in \Rb^{r_\pre \times (r-r_\pre)}$, where its entries are first independently sampled from a uniform distribution over $[0,1]$, and then its columns are normalized to sum to one; 
%
(iii) define $\bU_\pre = [\bA, \bA \bQ]$ as the concatenation of $\bA$ and $\bA \bQ$. 
%
By construction, $\bU_\pre$ has rank $r_\pre$ w.h.p., which we empirically verify.
%
Next, we define $\Ex[\bY_{\pre, \Ic^{(d)}}] = \bU_\pre \bV^\prime_{\Ic^{(d)}} \in \Rb^{T_0 \times N_d}$. 
%
Again by construction, we note that $\rank(\Ex[\bY_{\pre, \Ic^{(d)}}]) = r_\pre$ w.h.p., 
which we empirically verify. 
%
We then generate the model $w^{(n,d)} \in \Rb^{N_d}$ from a multivariate standard normal distribution, and define $\Ex[Y_{\pre, n}] = \Ex[\bY_{\pre, \Ic^{(d)}}] w^{(n,d)} \in \Rb^{T_0}$. 

\vspace{10pt} 
\noindent 
{\em Post-intervention data.} 
%
We choose $T_1 = 200$. 
%
We sample the post-intervention time factors as follows: 
%
(i) let $\bP \in \Rb^{T_1 \times T_0}$, where its entries are first independently sampled from a uniform distribution over $[0,1]$, and then its rows are normalized to sum to one; 
%
(ii) define $\bU_\post = \bP \bU_\pre \in \Rb^{T_1 \times r}$. 
We then define $\Ex[\bY_{\post, \Ic^{(d)}}] = \bU_\post \bV^\prime_{\Ic^{(d)}} \in \Rb^{T_1 \times N_d}$. 
%
To study the effect of the post-intervention period length, we will treat it as a variable. 
%
As such, we define $\Ex[\bY_{\post, \Ic^{(d)}}(\rho)] \in \Rb^{\rho T_1 \times N_d}$ as the first $\rho T_1$ rows of $\Ex[\bY_{\post, \Ic^{(d)}}]$, where  $\rho \in \{0.1, 0.2, \dots, 1.0\}$. 
%
For every $\rho$, we define $\theta^{(d)}_n(\rho)$ using $\Ex[\bY_{\post, \Ic^{(d)}}(\rho)]$ and $w^{(n,d)}$. 

\vspace{10pt} 
\noindent 
{\em Interpretation of data generating process.} 
%
We now motivate the construction of $\Ex[\bY_{\pre, \Ic^{(d)}}]$ and  $\Ex[\bY_{\post, \Ic^{(d)}}]$.
%
Recall that the SI framework allows potential outcomes from different interventions to be sampled from different distributions.
%
As such, we construct $\Ex[\bY_{\post, \Ic^{(d)}}]$ such that they follow a different distribution to that of $\Ex[\bY_{\pre, \Ic^{(d)}}]$. 
%
This allows us to study when the model learnt using pre-intervention data ``generalizes'' to a post-intervention regime generated from a different distribution. 
%
However, we note that by construction, Assumption \ref{assumption:subspace} holds w.h.p. between $\Ex[\bY_{\post, \Ic^{(d)}}(\rho)]$ and $\Ex[\bY_{\pre, \Ic^{(d)}}]$ for every $\rho$. 
%
We empirically verify all three conditions. 

\vspace{10pt} 
\noindent 
{\em Observations.} 
We generate $Y_{\pre, n}$ and $\bY_{\pre, \Ic^{(d)}}$ by adding independent noise entries from a normal distribution with mean zero and variance $\sigma^2 = 0.3$ to $\Ex[Y_{\pre, n}]$ and $\Ex[\bY_{\pre, \Ic^{(d)}}]$, respectively.
%
For every $\rho$, we generate $\bY_{\post, \Ic^{(d)}}(\rho)$ by applying the same additive noise model to $\Ex[\bY_{\post, \Ic^{(d)}} (\rho)]$.

\vspace{10pt} 
\noindent 
{\em Verifying assumptions.}
%
We note that our data generating process ensures that Assumptions \ref{assumption:sutva}, \ref{assumption:conditional_mean_zero},  \ref{assumption:noise} hold.
%
In addition, we empirically verify Assumptions \ref{assumption:boundedness} and \ref{assumption:spectra}.
%
Further, for Assumption \ref{assumption:form}, we note that our pre- and post-intervention (expected) potential outcomes associated with $\Ic^{(d)}$ were all generated using $\bV_{\Ic^{(d)}}$; thus, their variations only arise due to the sampling procedure for their respective latent time-intervention factors. 
%
%As such, Assumption \ref{assumption:form} holds. 
%
Given that $\Ex[Y_{\pre, n}]$ and $\theta^{(d)}_n(\rho)$ were both defined using $w^{(n,d)}$,  Assumption \ref{assumption:linear} holds. 
%
%In addition, we empirically verify that Assumption \ref{assumption:spectra} holds. 

\subsubsection{Simulation Setup} 
%
We perform $100$ iterations for each $\rho$. 
%
The potential outcomes, $\Ex[Y_{\pre,n}]$, $\Ex[\bY_{\pre, \Ic^{(d)}}]$, $\Ex[\bY_{\post, \Ic^{(d)}}(\rho)]$ are fixed, but the idiosyncratic shocks are re-sampled every iteration to yield new (random) outcomes. 
%
For each iteration, we use $(Y_{\pre, n}, \bY_{\pre, \Ic^{(d)}})$ to learn $\hw^{(n,d)}$, as given by \eqref{eq:pcr}. 
%
Then, we use $\bY_{\post, \Ic^{(d)}}(\rho)$ and $\hw^{(n,d)}$ to yield $\htheta^{(d)}_n(\rho)$, as given by \eqref{eq:si.2}.
%
The mean absolute errors (MAEs), $|\htheta^{(d)}_n(\rho) - \theta^{(d)}_n(\rho)|$ are plotted
in Figure \ref{fig:consistency}.  
%



% ASYMPTOTIC NORMALITY PART I 
\subsection{Asymptotic Normality: Subspace Inclusion Holds} 
%
In this section, we describe the setup for Section~\ref{sec:sim_normality1}.  

\subsubsection{Generative Model for Synthetic Data} 
%
We consider the binary $D=2$ intervention model. 
%
Our interest is in estimating $\theta^{(1)}_n$.
%
Our data generating process will be such that the pre- and post-intervention data will obey different distributions. 
%
Towards this, we choose $N_1 = |\Ic^{(1)} | = 400$ and $r = 15$.
%
We define $\bV \in \Rb^{N_1 \times r}$, where its entries are independently sampled from a standard normal.


\vspace{10pt} 
\noindent
{\em Pre-intervention data.} 
%
We choose $T_0 = 400$, and define the latent pre-intervention time factors under control as $\bU_\pre \in \Rb^{T_0 \times r}$, where its entries are sampled independently from a standard normal. 
%
Next, we define $\Ex[\bY_{\pre, \Ic^{(1)}}] = \bU_\pre \bV^\prime \in \Rb^{T_0 \times N_1}$. 
%
By construction, $\rank(\Ex[\bY_{\pre, \Ic^{(1)}}]) = r$ w.h.p., which we empirically verify. 
%
We then generate the model $ w^{(n,1)} \in \Rb^{N_1}$ from a standard normal, and define $\Ex[Y_{\pre, n}] = \Ex[\bY_{\pre, \Ic^{(1)}}] w^{(n,1)} \in \Rb^{T_0}$.
%
We define $\tw^{(n,1)} = \Ex[Y_{\pre, \Ic^{(1)}}]^{\dagger} \Ex[Y_{\pre, n}]$, where $\dagger$ is the pseudo-inverse. 
%

\vspace{10pt} 
\noindent
{\em Post-intervention data.} 
%
We choose $T_1= 20$, and generate post-intervention time factors under $d=1$ as follows: 
%
We define $\bU_{\post} \in \Rb^{T_1 \times r}$, where its entries are independently sampled uniformly over $[-\sqrt{3}, \sqrt{3}]$.
%
We then define $\Ex[\bY_{\post, \Ic^{(1)}}] = \bU_\post \bV^\prime \in \Rb^{T_1 \times N_1}$.
%
Finally, we define $\theta^{(1)}_n$ using $\Ex[\bY_{\post, \Ic^{(1)}}]$ and $w^{(n,1)}$. 

\vspace{10pt}
\noindent
{\em Interpretation of data generating process.} 
%
%We motivate our data generatin
%the construction of $\Ex[\bY_{\pre, \Ic^{(0)}}]$, $\Ex[\bY_{\post, \Ic^{(0)}}]$, $\Ex[\bY_{\post, \Ic^{(1)}}]$.
%
We note $\Ex[\bY_{\pre, \Ic^{(1)}}]$ and $\Ex[\bY_{\post, \Ic^{(1)}}]$ follow different distributions to reflect that the pre- and post-intervention potential outcomes are associated with different interventions; the former with $d=0$ and the latter with $d=1$. 
%
However, by construction, $\Ex[\bY_{\post, \Ic^{(1)}}]$ satisfies Assumption \ref{assumption:subspace} with respect to $\Ex[\bY_{\pre, \Ic^{(1)}}]$ w.h.p., 
which we empirically verify. 

\vspace{10pt}
\noindent
{\em Observations.} 
%
We generate $Y_{\pre, n}$ and $\bY_{\pre, \Ic^{(1)}}$ 
by adding independent noise from a normal distribution with mean zero and 
variance $\sigma^2 = 0.5$ to $\Ex[Y_{\pre, n}]$ and 
$\Ex[\bY_{\pre, \Ic^{(1)}}]$, respectively. 
%
We generate $\bY_{\post, \Ic^{(1)}}$ by applying the same additive 
noise model to $\Ex[\bY_{\post, \Ic^{(1)}}]$.
%

\vspace{10pt}
\noindent
{\em Verifying assumptions.} 
%
As before, Assumptions \ref{assumption:sutva} to \ref{assumption:spectra} hold by construction. 

\subsubsection{Simulation Setup} 
%
We perform 5000 iterations, where $\Ex[Y_{\pre, n}], \Ex[\bY_{\pre, \Ic^{(0)}}]$, $\Ex[\bY_{\post, \Ic^{(1)}}]$ are fixed throughout, but the idiosyncratic shocks are re-sampled to generate new (random) outcomes. 
%
Within each iteration, we first use  $(Y_{\pre, n}, \bY_{\pre, \Ic^{(1)}})$ to fit $\hw^{(n,1)}$, as in \eqref{eq:pcr}. 
%
Next, we use $\bY_{\post, \Ic^{(1)}}$ and $\hw^{(n,1)}$ to yield $\htheta^{(1)}_n$, as in \eqref{eq:si.2}.  
%
The resulting histogram is displayed in Figure~\ref{fig:good}. 



% ASYMPTOTIC NORMALITY PART I 
\subsection{Asymptotic Normality: Subspace Inclusion Fails}
%
Next, we describe the setup for Section~\ref{sec:sim_normality2}. 

\subsubsection{Generative Model for Synthetic Data} 
%
We continue analyzing the binary $D=2$ intervention model. 
%
We let $N_1 = 400, r = 15$, and generate %the latent unit factors associated with $\Ic^{(1)}$ as 
$\bV_{\Ic^{(1)}} \in \Rb^{N_1 \times r}$ by independently sampling its entries from a standard normal. 

\vspace{10pt}
\noindent
{\em Pre-intervention data.}
%
We choose $T_0 = 400$ and $r_\pre = 12$. 
%
We construct $\Ex[\bY_{\pre, \Ic^{(1)}}]$ using $\bV_{\Ic^{(1)}}$
identically to that in Section \ref{ssec:empirics_consistency_model}, such that $\rank(\Ex[\bY_{\pre, \Ic^{(1)}}]) = r_\pre$ w.h.p., which we empirically verify. 
%
As before, we generate $w^{(n,1)} \in \Rb^{N_1}$ from a standard normal
and define $\Ex[Y_{\pre,n}] = \Ex[\bY_{\pre, \Ic^{(1)}}] w^{(n,1)} \in \Rb^{T_0}$, as well as 
%
$\tw^{(n,1)} = \Ex[\bY_{\pre, \Ic^{(1)}}]^{\dagger} \Ex[Y_{\pre, n}]$. 
 

\vspace{10pt}
\noindent
{\em Post-intervention data.} 
%
We choose $T_1=20$, and define the post-intervention time factors under $d=1$ as $\bU_\post \in \Rb^{T_1 \times r}$, where its entries are sampled independently from a standard normal. 
%
Next, we define $\Ex[\bY_{\post, \Ic^{(1)}}] = \bU_\post \bV^\prime_{\Ic^{(1)}} \in \Rb^{T_1 \times N_1}$. 
%
By construction, $\rank(\Ex[\bY_{\post, \Ic^{(1)}}]) = r$ w.h.p., which we empirically verify. 
%
Since $r_\pre < r$, Assumption \ref{assumption:subspace} fails between $\Ex[\bY_{\pre, \Ic^{(1)}}]$ and $\Ex[\bY_{\post, \Ic^{(1)}}]$. 
%
We define $\theta^{(1)}_n$ using $\Ex[\bY_{\post, \Ic^{(1)}}]$ and $w^{(n,1)}$. 

\vspace{10pt}
\noindent
{\em Observations.} 
%
We generate $Y_{\pre, n}$ and $\bY_{\pre, \Ic^{(1)}}$ by adding independent noise from a normal distribution with mean zero and variance $\sigma^2 = 0.5$ to $\Ex[Y_{\pre, n}]$ 
and $\Ex[\bY_{\pre, \Ic^{(1)}}]$, respectively. 
%
We generate $\bY_{\post, \Ic^{(1)}}$ by applying the same noise model to $\Ex[\bY_{\post, \Ic^{(1)}}]$. 
%

\vspace{10pt}
\noindent
{\em Verifying assumptions.} 
%
As before,  Assumptions \ref{assumption:sutva} to  \ref{assumption:spectra} hold by construction. 

\subsection{Simulation Setup}
%
We perform 5000 iterations, where $\Ex[Y_{\pre,n}], \Ex[\bY_{\pre, \Ic^{(1)}}]$, $\Ex[\bY_{\post, \Ic^{(1)}}]$ are fixed, but the idiosyncratic shocks are re-sampled. 
%
In each iteration, we use $(Y_{\pre, n}, \bY_{\pre, \Ic^{(1)}})$ to fit $\hw^{(n,1)}$, and then use $\bY_{\post, \Ic^{(1)}}$ and $\hw^{(n,1)}$ to yield $\htheta^{(1)}_n$. % as in \eqref{eq:si.2}. 
%
The resulting histogram is displayed in Figure \ref{fig:bad}.


==> content/synth_a_b.tex <==
\section{Implications of \SI~Toward Experiment Design}\label{sec:synth_a_b}
%
Motivated by the empirics in Section \ref{sec:empirics}, we discuss how the \SI~estimator can be used to develop novel experiment designs that are more data-efficient. 
%
We name our design {\em synthetic A/B testing}.

\subsection{Description} 
%
To recap, we look to develop an experiment design that estimates $N \times D$ causal parameters, $\{\theta^{(d)}_n : (n, d) \in [N] \times [D] \}$, from far fewer than $T \times N \times D$ outcomes. 
%
Specifically, our task is two-fold: 
%
(i) select $\Dc \subset [T] \times [N] \times [D]$ outcomes to observe; 
%
(ii) estimate the causal parameters of interest from $\Dc$.
%
Ideally, $|\Dc|$ is as small as possible to achieve the required estimation error. 

In what follows, we discuss two variants of the synthetic A/B testing experiment design. 
%
Appendix \ref{sec:a_b_test_multiple} proposes an experiment design when units (e.g., customer sub-populations) can be simultaneously observed under multiple interventions.
%
Appendix \ref{sec:a_b_test_individual} proposes an experiment design when units (e.g., individual customers) are restricted to be observed under a single intervention. 

% Simultaneous 
\subsubsection{Simultaneous Interventions.} \label{sec:a_b_test_multiple}
%
Suppose units can be simultaneously observed under multiple interventions.
%
For example, e-commerce platforms can randomly choose individual customers from the same customer sub-population to receive different discounts simultaneously.
%
In line with the validation study of Section \ref{sec:empirics}, we propose a simple experiment design where each unit is observed under exactly two interventions: control (denoted as $d=0$) and one of the other $D-1$ interventions. 
%
Specifically, all $N$ units are randomly partitioned into $D-1$ groups of roughly equal size. 
%
Then, all units within a group are assigned the same intervention. 
%
By design, we observe $T \times N \times 2$ out of the $T \times N \times D$ entries in the potential outcomes tensor $\bY$. 
%
See Figure \ref{fig:o2_later} for a visual depiction of the observation pattern associated with our design.  
%
\begin{figure}[t!]
	\centering 
	\begin{subfigure}[b]{0.35\textwidth}
		\centering 
		\includegraphics[width=\linewidth]
		%{images/mode2.png}
		{images/o2.jpg}
		\caption{Simultaneous interventions.} 
		\label{fig:o2_later}
	\end{subfigure} 
	%
	\begin{subfigure}[b]{0.33\textwidth}
		\centering 
		\includegraphics[width=\linewidth]
		%{images/mode1.png}
		{images/o1.jpg}
		\caption{Single intervention.} 
		\label{fig:o1_later} 
	\end{subfigure} 
	\qquad
	\caption{Observation pattern associated with our synthetic A/B testing design, where observed outcomes are represented by colored blocks while missing entries are represented by white blocks. 
	}
	\label{fig:observations_later} 
\end{figure}

To estimate the causal parameters from our observations, we adopt the following strategy for each intervention $d$: 
%
\begin{enumerate}
	\item[(a)] for all $n \in \cI^{(d)}$, we estimate $\theta^{(d)}_n$ with $\htheta^{(d)}_n = T^{-1} \sum_{t=1}^T Y_{tnd}$; 
	
	\item[(b)] for all $n \notin \cI^{(d)}$, we estimate $\theta^{(d)}_n$ via the \SI~estimator described in Section~\ref{sec:algo}. 
\end{enumerate}
%
Observe that $\Tc_\pre = \Tc_\post = [T]$ in our setting of interest. 
 
% SINGLE INTERVENTION 
\medskip
\subsubsection{Single Intervention.} \label{sec:a_b_test_individual}
%
Now, suppose each unit can only be observed under a single intervention for any measurement.
%
In our e-commerce example, this corresponds to individual customers---rather than customer sub-populations as in Section~\ref{sec:a_b_test_multiple}---representing our units. 
%
Unlike Section~\ref{sec:a_b_test_multiple}, $\Tc_\pre$ and $\Tc_\post$ will now correspond to different time points. 
%
Without loss of generality, let $\Tc_{\epre} = \{1, \dots, T - T_1 \}$ and $\Tc_{\epost} = \{T- T_1 + 1, \dots, T\}$. 

%
We propose the following experiment design. 
%
For each $t \in \Tc_{\pre}$, assign control ($d=0$) to all $N$ units. 
%
For $t \in \Tc_{\post}$, assign one of the $D$ interventions to each unit such that $N_d \approx N/D$ for all $d$. 
%
Accordingly, we observe $T \times N$ out of the $T \times N \times D$ entries in the potential outcomes tensor $\bY$. 
%
The natural trade-off between this setting compared to that in Appendix~\ref{sec:a_b_test_multiple} is that we cannot estimate the outcomes for all $T$ measurements but rather only for those in $\Tc_\post$.
%
See Figure \ref{fig:o1_later} for a visual depiction of the observation pattern induced by this design. 
%

To estimate the causal parameters from our observations, we adopt the following strategy for each intervention $d$: 
%
\begin{enumerate}
	\item[(a)] for all $n \in \cI^{(d)}$, we estimate $\theta^{(d)}_n$ with $\htheta^{(d)}_n = T_1^{-1} \sum_{t \in \Tc_\post} Y_{tnd}$; 
	
	\item[(b)] for all $n \notin \cI^{(d)}$, we estimate $\theta^{(d)}_n$ via the \SI~estimator described in Section~\ref{sec:algo}. 
\end{enumerate}

% FACTORIAL DESIGN
\subsection{Factorial Design} 
%
Suppose there are $K$ ``types'' of interventions designed to have an effect on a common set of outcomes. 
%
Continuing the e-commerce application in Section \ref{sec:empirics}, imagine that along with offering customers different discounts, the e-commerce platform also had other levers to increase engagement levels such as sending marketing emails and offering different versions of the product to its customers.
%
In this case, we have $K = 3$. 
%
Now, suppose there were $L$ different versions of each of the $K$ interventions. 
%
In the case of discounts, there were $L = 4$ versions corresponding to $\{0\%, 10\%, 30\%, 50\%\}$.
%
This yields $D = L^K$ possible interventions.
%
Since $D$ grows exponentially in $K$, running factorial design experiments can be massively expensive even for small $K$ and $L$.


Our theoretical results imply that our proposed synthetic A/B testing framework can accurately estimate the treatment effect of all $L^K$ interventions on a {\em unit-by-unit} basis while observing each unit under at most $2$ interventions, provided $N$ is large enough.
%
The tensor factor model in Assumption \ref{assumption:form} does not make any assumption about how the $L$ types of interventions interact with each other as it only posits that the latent factor $v_n$ associated with each unit is invariant across the $L^K$ interventions.
%
This is in contrast to the literature on factorial design experiments where, for example, one posits that there are only pairwise interactions between the $K$ different interventions \citep{george2005statistics}.
%
Indeed, finding ways to incorporate structure across combinations of interventions without requiring some number of units to undergo each of the $L^K$ interventions into the \SI~framework is left as interesting future work.
%








